A $b$-baryon sonata

LHCb is one of the four experiments at the Large Hadron Collider (CERN), dedicated to the study of b-hadrons. Throughout my research, I studied in particular b-baryons which are abundantly produced at the LHCb. My habilitation summarises the studies of fundamental properties of these particles within the Standard Model. In particular, I discuss both lifetime and mass measurements. This work is followed by a search of New Physics using a Lepton universality test. Finally, I discuss my contribution to the upgrade detectors of the LHCb experiment in particular those related to the calorimeter and the scintillator fibre tracker.

==> apprentices.tex <==
\chapter*{Apprentices}
An HDR would make little to probably no sense without the participation of students.
I had the pleasure to supervise and co-supervise many bachelor (L3) and master (M1 or M2) students since I started working at CNRS in 2012. I don't mention in this section the contribution of my PhD students Renato Quagliani and Vitalii Lisovskyi  as they each produced almost 300 pages of material describing their work~\cite{Quagliani:2296404}, \cite{Lisovskyi:2699822}. 
They all played very different roles and contributed to many areas of my research activities for example, they helped me to kick-start physics analyses, learn new techniques, methods or software, study the feasibility of a measurement, address a specific analysis point. I would like to thank all of them for their enthusiasm and energy. I would like also to thank Carla Marin Benito \& S\'ebastien Descotes-Genon who shared some of the supervision with me.  
%------------------------------

\subsection*{Kevin de Vasconcelos Corga 2013/M1}
With Kevin we evaluated the expected statistical uncertainty on $\Delta \Gamma_d$ and $\tau_\Bz$ using LHCb 2011 and 2012 datasets. 
Kevin wrote a new fitting program which permitted to access the observables of interest in a simulatanous way from \Bz\to\jpsi \KS and \Bz\to\jpsi\Kstarz signal events. He also made an extrapolation for the LHCb Upgrade. For this study, there was no special treatment of the \KS tracks, both types of track categories were accounted for and each of them had their own decay time acceptance.


\subsection*{Ilham Dami  2015/L3 }
With Ilham we stated the lepton universality analysis with \Lb decays. During her internship, Ilham studied the shape of the rare electron mode using simulated samples of $\Lb \to \Lambda (1520)e^{+}e^{-}$ decays.  We also had a look at multivariate selections for this decay mode, she used the scikit learn software and we played with the various algorithms and optimisation techniques~\cite{scikit-learn}. 

\subsection*{Rabah Abdul Khalek 2016/M1}
Rabah's internship happened during a time where I was working on the software of the scintillator fibre tracker for the LHCb Upgrade. Trying to reduce the processing time and optimise the algorithms was a priority. 
Using dedicated tools such as {\tt Valgrind}, Rabah identified that a significant amount of processing time was spent in the first loop making combinations from hits from \xlayers. He rewrote part of this code in a smarter way and this allowed to reduce the processing time in this step by a factor two. Later on, he gave a try to using a Neural Network in the suppression of the ghosts track combinations inside the algorithm. 
With this improvement the ghost rate was reduced by a factor two. 



\subsection*{Florian Mercier - 2017/L3} 
Co-supervised with S\'ebastien Descotes-Genon.\\
During three years, I shared a course called "introduction to particle physics" for  second year bachelor students. Amongst my students Florian was probably the most curious one, and he asked me for advice. He wanted to do an internship working on a "theory" project but he was worried to end up only reading papers and making photocopies. After discussing with S. Descotes-Genon, we agreed to share his supervisor and investigate what would be the impact of measuring properties of $\Lb\to \Lambda(1520) \ell^{+}\ell^{-}$ decays in global fits. 
Florian used {\tt flavio} a python based package for global flavour fits~\cite{Straub:2018kue}. 
A few assumptions had to me made given that no form factors were computed for this decay, he used approximations suggested in arXiv:1102.00897 based on quark models and Heavy Quark Effective theory and produced constraints on the Wilson coefficients $C_{9}$ and $C_{10}$. 


\subsection*{Mathieu  Markovitch \&  Corentin van Den Broek D'obrenan -  2019/L3 }
Co-supervised with Carla Marin Benito. \\
The work of Mathieu and Corentin was based on arXiv:1807.01643. 
Mathieu studied the impact of the radiative decay $B_s\to f_1(1420)\gamma$ on the Wilson coefficient $C_7^{\prime}$ associated with right-handed currents in $\bquark\to\squark$ transitions using the {\tt flavio} package.
The final state $B_s\to f_1(1420) (\to K K \piz) \gamma$ is quite challenging to reconstruct at LHCb. Corentin used multivariate approches from the scikit learn software to evaluate the possibility of seeing this signal in the LHCb data.


\subsection*{Felicia  Volle - 2019/M2}
Co-supervised with Carla Marin Benito. \\
The $m(\proton\kaon)$ spectrum from $\Lb\to pK \ell^{+}\ell^{-}$ decays has never been measured outside of the $\jpsi$ region, ultimately it will be needed to know the resonant structure of the hadronic part of the rare modes to be able to compare any result to theoretical predictions and this will be possible when enough data will be analysed. 
One can use the region around $q^{2}=0$, where the photon is produced on shell to perform such a study. As part of her internship, Felicia worked on a selection using a multi-variable method to isolate $\Lb\to pK\gamma$  decays.
She showed that one can expect to have about 1'000 signal candidates in 2012 data collected by LHCb. 

\subsection*{Anja Beck - 2019/M2 }  
Co-supervised with Carla Marin Benito. \\ Anja is enrolled at the University of Dortmund in Johannes Albrecht's group. She spent six months in our group at IJCLab as part of an Erasmus program.
Anja's work is a follow up of Felicia's one. She first  investigated the shape of the angular acceptance and resolution.   Anja dived in the helicity formalism needed to perform the amplitude analysis of
$\Lb\to pK\gamma$.  This work is now documented in arXiv:2002.02692 and submitted to JHEP. The amplitude fit that she is developing is based on the TensorFlow software. She already has a version of the fit which gives sensible results of the fractions for the different $\Lambda^{*}$ resonances, using the legacy Run 1/2 LHCb datasets. 





==> detector.tex <==
\chapter{Allegretto}
\epigraph{\textit {``Don't you know that Rome wasn't built in a day"}}{Morcheeba}



\section{The LHCb detector }
\label{sec:detector}
The LHCb detector~\cite{LHCb}, shown in Figure~\ref{fig:lhcb}, was designed to study the asymmetry between matter and anti-matter, and search for physics beyond the SM in \bquark-hadron decays. 
It turned out that the excellent performance of the detector was such that the physics program  was extended very rapidly to explore also charm, electroweak, and, more recently, heavy ion physics. 
 

\begin{figure}[ht!]
  \centering
  \includegraphics[width=0.55\textwidth]{figs/detector/lhcb/lhcb.pdf}
  \caption{The LHCb detector~\cite{LHCb}.}
  \label{fig:lhcb}
\end{figure}
LHCb  is a single-arm spectrometer located at the interaction point (IP) 8 of the LHC.
The choice of detector geometry is justified by the fact that both \bquark and $\bar{b}$ hadrons are predominantly
produced in the same forward or backward cone.  If our collaboration had the budget of the ministry of defence we would probably have built two LHCb detectors, to catch both the forward and backward pairs.  Charged tracks are detected by a vertex locator near to the
IP, and their momenta and charge are subsequently determined with tracking stations (TT, T1, T2 and T3)
either side of a magnet providing an integrated field of 4 Tm.  
The tracking efficiencies were found to be $\sim 96\%$  for $\jpsi\to \mup \mu^{-}$ in the momentum range $5 \gevc < p < 200 \gevc$. Ring imaging Cherenkov (RICH) counters
are used to distinguish kaons, pions and protons.
An excellent hadron identification is crucial for a flavour experiment\footnote{For instance, for a requirement on the \kaon-\pion separation, $\Delta log {\cal L}(\kaon - \pion) > 0$, when averaging over the momentum range 2-100 GeV/c one finds the kaon efficiency to be $\sim95\%$ with a pion misidentification rate of $\sim 10\%$.}, for example the measurement of $\CP$ asymmetries in $B_{d,s}^{0}\to \pi\pi, \kaon\kaon, \pion\pion$ decays.  
Electromagnetic and hadronic calorimeters (ECAL and HCAL),
together with an instrumented preshower (SPD/PS) system, provide measurements of the energies of neutral particles
as well as electrons. Finally, muons are identified with a dedicated detection system (M1-M5).
The  vertex locator provides precise information on the origin of the tracks and the  tracking stations are essential to measure the momenta of the particles involved in the decay of the particles of interest.
This gives extremely powerful information to reject background, since signal tracks \ie secondary particles produced by the particles of interest, must originate from common vertices that are displaced from the primary vertex of the LHC proton-proton collision, due to the non-negligible lifetimes of the decaying bottom hadrons (${\cal O}(1)$ ps), whereas the largest potential source of background is from random combinations of tracks that originate from the primary vertex. 
The LHCb trigger is a key to the success of the experiment. It operates in two stages.  A hardware trigger based on the information provided by the calorimeters and the muon chambers reduces the frequency of events from the LHC beam crossing rate of up to 40 MHz to a
rate of 1 MHz at which the entire detector can be read out. 
The subsequent high-level software trigger stage  was responsible for reducing the output rate to a level at which data can be written to permanent storage.
This rate evolved significantly between Run 1 and Run 2, reaching 12.5 kHz at the end of Run 2. Detailed discussion of the  performances of the LHCb detector can be found in Ref.~\cite{Aaij:1978280}.
The Run naming convention and the schedule of the LHC are defined in Table~\ref{tab:lhc}.
\begin{table}[!ht]
\centering
\begin{tabular}{c|c|c|c|c|c|c}
Run 1  & LS1 &  Run 2 & LS2 & Run 3  & LS3 & Run 4... \\
\hline
\cellcolor{blue!25}  2010-2012 & \cellcolor{yellow}  2013-2015&\cellcolor{blue!25}   2015-2018& \cellcolor{yellow} 2018 - 2020 & \cellcolor{blue!25}  2021-2024 &\cellcolor{yellow}   2025 - 2027 & \cellcolor{blue!25}      2027 - ....\\
\end{tabular}
\caption {LHC schedule. The data taking period are highlighted in blue,  the technical stops are highlighted in yellow.}
\label{tab:lhc}
\end{table}


The LHCb detector is currently undergoing its first major upgrade to allow for data taking at $2\times 10^{33}$cm$^{-2}$s$^{-1}$ in 2021, a factor five increase compared to earlier runs. All the tracking system will be replaced~\cite{Bediaga:1443882}. 
The vertex locator strips will be replaced by pixel detectors~\cite{Collaboration:1624070}, and the TT will be upgraded to an Upstream Tracker (UT) with a larger acceptance around the beam pipe. The central trackers will be replaced with a scintillating fibre tracker (SciFi). 
Furthermore, the entire electronics  will be replaced to allow the detector to be read out at the proton-proton collision rate, and to send the data to be processed online in the high level trigger. In order to maximise the physics output of the experiment, the philosophy of the collaboration has been to perform full track reconstruction, including particle identification and track fitting, as early as possible in the data processing.  

I have been involved in two upgrade projects. With my former PhD student Renato Quagliani~\cite{Quagliani:2296404}, whom I co-supervised with Patrick Robbe and colleagues from LPNHE in Paris, Pierre Billoir and Francesco Polci, we developed a  pattern recognition algorithm that we baptised {\tt Hybrid Seeding}. The aim of this tracking algorithm is to reconstruct track segments using only in the information of the SciFi, enabling later the reconstruction of long-lived particles such as  \KS, \Lz or more exotic ones, like dark photon candidates.   This algorithm and its performance are discussed in  Section~\ref{sec:tracking}. I am also involved in a hardware project for the calorimeter, where I am responsible for a control board designed by  O.Duarte and A.Saussac. The purpose of this board is to distribute information from the central LHCb system  such as the 40 MHz clock and propagate it to the calorimeter front-end boards. The design of this board is described Section~\ref{sec:calorimeters}.  


\section{Pattern recognition}
\label{sec:tracking}
The LHCb upgrade tracking algorithms rely on three detectors: the vertex locator, the upstream tracker and the scintillating fibre tracker. Figure~\ref{fig:tracktypes} shows the different types of tracks produced by the reconstruction; their somewhat jargonic classification can be found in Table ~\ref{tab:tracksEff}. 
\begin{figure}
\centering
\includegraphics [width=0.5\textwidth]{figs/detector/tracking/tracking.png}
\caption{Track types in the LHCb Upgrade.}
\label{fig:tracktypes}
\end{figure}

The SciFi tracker~\cite{Collaboration:1647400} is composed of three tracking stations,  T1, T2, T3. Each station is composed of four layers, separated by air-filled gap of 50 \mm, oriented in the so called \textit{stereo} configuration (\textit{x-u-v-x}). The fibre mats in the first and fourth \xlayer (within the same station) are vertically oriented, \ie the fibre mats are parallel to the \textit{y} axis of the laboratory frame. Therefore, the read-out of a \xlayer provides the direct measurement of the $x^{track}(z_{layer})$ position. But no information at all about the \textit{y} can be  directly extracted.  
The second (\textit{u}) and the third (\textit{v}) layers are identical to the \xlayer, but their fibre mats are tilted with respect to the \xlayer by $+5^{\circ}$ and $-5^{\circ}$ respectively. The read-out of the \uvlayers provides the \textit{u} and \textit{v} stereo coordinates, which are used to extract the information on the \textit{y-z} plane motion of the particles. 

The SciFi tracker benefits from a  good uniformity whereas the former central tracking system, was based on different technologies, mechanical supports \etc. 
This ensures that the fraction of particles that survive the passage through the SciFi Tracker is quite high. The fraction was found to be 96.9\% for hadrons, 93.9\% for electrons and 95.2\% for photons.
With the SciFi, a difficulty was  introduced  by the absence of a $y$- segmentation in the tracker. 
This feature makes the track finding close to the beam pipe, where the detector occupancy is the highest, quite challenging, and the impact of the loss of light propagation in the fibres, a particular problem.  Renato worked out a way around this. From the expected $y$-position of a traversing track based on the information from the \xlayers and the stereo ones, he figured out  a way  to tune the hit requirements of the tracks  according to the expected light attenuation in the SciFi fibres, which reduced significantly the fake (or ghost) rate.


The decay rates and topologies considered for the LHCb Upgrade are very broad~\cite{Bediaga:1443882}. 
They vary from rare decays, such as the very rare $B_s^{0}\to \mup\mu^{-}$ mode or the radiative mode $\Lb \to \Lz \gamma$, to multi-track final states such as $B_s^{0}\to D_s^{+} (\to \Kp\Km\pip)D_s^{-} (\to \Kp\Km\pim)$. One has also to take into account from the spread of the momentum ranges of these particles, from the  very soft tracks like the pions from $D^*$ decays all the way to the hard ones from $W$ and $Z$ decays.  
With this in mind, the algorithm was designed to reach a good compromise in the holy tracking trinity: high tracking efficiencies and low fake rate and small processing time. 
 
 The main idea behind the {\tt Hybrid Seeding} is to  progressively clean the tracking environment by first finding the tracks which are easier to reconstruct, and then searching for those with more complicated trajectories or signatures using the left-over hits. 

Some of the improvements reached were achieved thanks to an update of the track parametrisation, an  optimisation of the search windows and a redesign of the loops over the hit containers. 
The rethinking of recovery routines permitted to improve the low momentum track efficiency and the robustness of the algorithm.


\begin{table}[!ht]  
  \centering
  \resizebox{0.8\textwidth}{!}{              
    \begin{tabular}{l|l}         
    \toprule                            
      Name & Property \\ \midrule %\hline  
      \textit{hasT} & \reconstructible in \scifi \\                                                         
      \UT + \scifi & \reconstructible in \scifi and \UT \\                                                                  
      \textit{noVelo} & not \reconstructible in the \velo \\                                                                
      \textit{long} &  \reconstructible in \velo and \scifi \\                                                              
      \textit{strange} & daughter of a strange particle ( \KS, \Lz, ..) \\                                                  
      \textit{from B} & belong to the decay chain of a $b$ hadron \\                                                         
      \textit{from D} & belong to the decay chain of a $c$ hadron \\
      \bottomrule
    \end{tabular}  }                                                         
  \caption{\small Sub-selections used by the  performances indicators.}\label{tab:tracksEff}                            
\end{table}  

The results obtained from these studies are summarised in Table ~\ref{tab:efficienciessample1} and Figure~\ref{fig:Sample2Effstrange}. They make clear that the \HybridAlgo performs significantly better than the first implementation of the prototype algorithm  referred to in this text as  \OldAlgo. A significant improvement is achieved in all the fields:
\begin{itemize}
\item The \ghostrate is  reduced by a factor two with respect to the old seeding version (even when averaged for the events), and the efficiencies are significantly larger.
\item The \treffs are  significantly improved for all the track categories, especially for lower $p$ and $p_{T}$ tracks ($\sim$20 \%), while for higher $p$ a gain of 4-6 \% is achieved.
\item The \clone killing which allows to remove duplicate candidates is more efficient than the  previous algorithm. This is achieved thanks to a more accurate track comparison and  to the internal sorting of the hits, which allows a better track-to-track comparison. 
\item The \textit{timing} of the \HybridAlgo is significantly improved with respect to \OldAlgo, by almost a factor 3-4 on average (depending on the detector occupancy level), as shown in Table~\ref{tab:timing}. 
\end{itemize}

In other words, \HybridAlgo is more robust against busy events with respect to the \OldAlgo. Timing comparisons have been achieved running both the algorithms on the same machine (a standard lxplus machine SLC6 in 64-bit mode) and we also quote the timing of the \textit{forward tracking} algorithm (as a reference value) in the so called best tracking sequence stage, \ie, the configuration aiming to find all \textit{long} tracks in the event.


\begin{table}[!htbp]
\centering
\resizebox{1.0\textwidth}{!}{
  \begin{tabular}{l|cc|c|c|c}
   \toprule
    Machine speed      &                   & Algorithm                        & Avg. time            & Min. time & Max. time \\ 
    $n\cdot$ 2.8 GHz Xenon&                          &        & [$\frac{ms}{evt.}$] & [$\frac{ms}{evt.}$] & [$\frac{ms}{evt.}$] \\ \midrule
%    \multirow{3}{*}{2.76}& \multirow{3}{*}{1}       &  \texttt{Forward Tracking Best}   & 29.95& 0.11 & 612.1 \\
  %                       &                          &  \OldAlgo                         & 72.75& 0.15 & 1770.0\\ 
    %                     &                          &  \HybridAlgo                      & 23.53& 0.24 & 589.4 \\ \midrule

   \multirow{3}{*}{2.79}& \multirow{3}{*}{}       &  \texttt{Forward Tracking Best}   & 48.62 &0.30&  1271.4 \\
                       &                          &  \OldAlgo                         & 150.95&1.86& 6069.0 \\ 
                       &                          &  \HybridAlgo                      & 46.80 &0.70& 1239.1 \\ \midrule
%
%    \multirow{3}{*}{2.99}& \multirow{3}{*}{3}       &  \texttt{Forward Tracking Best}   &30.16 &0.20 &1013.4 \\
%                       &                          &  \OldAlgo                         &79.44 &0.91 &2042.9 \\ 
%                       &                          &  \HybridAlgo                      &22.30 &0.37 &662.7 \\ \bottomrule

  \end{tabular}}
  \caption{Average, maximum and minimum timing of the algorithms for the different samples. Timing performances are also quoted with respect to the \textit{forward} tracking used for the upgrade.}\label{tab:timing}
  \label{tab:efficienciessample1}
\end{table}

  \begin{table}[!htbp]
  \centering
      \resizebox{0.8\textwidth}{!}{
        \begin{tabular}{l|c|c}\toprule
          \multirow{2}{*}{Track type } &\multicolumn{2}{c}{\textit{Sample 2}}                               \\ \cline{2-3}
                                       &\OldAlgo     & \HybridAlgo  \\
                                       & $\epsilon$ (\clonerate)         & $\epsilon$ (\clonerate)         \\  
         \midrule
          \textit{hasT}                                     &(53.5 $\pm$ 0.1)(3.5) $\%$  &(66.6 $\pm$ 0.1)(0.0) $\%$  \\
          \textit{long}                                     &(78.4 $\pm$ 0.1)(3.3) $\%$  &(92.1 $\pm$ 0.1)(0.0) $\%$  \\
          \textit{long} $P>5$\gevc                          &(87.5 $\pm$ 0.1)(2.6) $\%$  &(95.4 $\pm$ 0.4)(0.0) $\%$  \\
          \textit{long from B}                              &(80.4 $\pm$ 0.6)(2.7) $\%$  &(93.0 $\pm$ 0.3)(0.0) $\%$  \\
          \textit{long from B} $P>5$\gevc                   &(88.5 $\pm$ 0.5)(2.3) $\%$  &(95.9 $\pm$ 0.1)(0.0) $\%$  \\
          \textit{long from B or D}                         &(80.7 $\pm$ 0.2)(2.7) $\%$  &(93.3 $\pm$ 0.1)(0.0) $\%$  \\
          \textit{long from B or D} $P>5$\gevc              &(89.3 $\pm$ 0.2)(2.3) $\%$  &(95.9 $\pm$ 0.1)(0.0) $\%$ \\
          \UT+\scifi \textit{strange}                       &(76.3 $\pm$ 0.1)(3.3) $\%$  &(91.8 $\pm$ 0.1)(0.0) $\%$  \\
          \UT+\scifi \textit{strange} $P>5$\gevc            &(88.8 $\pm$ 0.1)(2.5) $\%$  &(95.7 $\pm$ 0.1)(0.0) $\%$  \\
          no\velo+\UT+\scifi \textit{strange}               &(76.8 $\pm$ 0.2)(3.3) $\%$  &(91.3 $\pm$ 0.1)(0.0) $\%$  \\
          no\velo+\UT+\scifi \textit{strange} $P>5$\gevc    &(88.7 $\pm$ 0.2)(2.7) $\%$  &(95.6 $\pm$ 0.1)(0.0) $\%$  \\
          \bottomrule \toprule
          \ghostrate                                        & (37.3 $\pm$ 0.1)$\%$     &(19.4 $\pm$ 0.1) $\%$     \\
          \ghostrate (evt.avg)                              & 21.6 $\%$               &   11.2  $\%$            \\  
          \bottomrule \toprule
          \hitpurity                                        & 98.9 $\%$                &   99.6 $\%$             \\
          \hitefficiency                                    & 93.6 $\%$                &   95.4 $\%$             \\
          \bottomrule
        \end{tabular}}\caption{Tracking performance comparison between the \OldAlgo and the \HybridAlgo algorithms.}\label{tab:efficienciessample2}
\end{table}

\begin{figure}
\begin{center}
 \includegraphics[angle=90,origin=c]{figs/detector/tracking/Sample2_UT+T_strange.pdf}
    \caption{\small \textit{Tracking efficiency} distributions, selecting tracks having hits in the \UT and the \scifi and being daughters of long-lived strange particles, such as $K^{0}_{S}$ or $\Lambda^{0}$. The efficiencies obtained with the \HybridAlgo (blue) algorithm are on average  $\simeq$12$\%$ better than the ones from the \OldAlgo.}
    %sample 2 for $B_s\phi(\Kp\Km)\phi (\Kp\Km)$
    \label{fig:Sample2Effstrange} 
\end{center}
  \end{figure}
  
 \newpage
The performance quoted in this section have been obtained with a description of the SciFi geometry which was not final. However, even with more refined versions of the geometry, which were later made available, the overall conclusions of this work remain unchanged.  The  {\tt Hybrid Seeding} algorithm has continued to evolve, and further improvements have been achieved. More recently, the focus of the efforts has been towards improving the reconstruction electrons at low momenta. 
  
  
  \section{Calorimeters}
  \label{sec:calorimeters}

 As part of the first phase of the LHCb upgrade and the calorimeters upgrade in particular, both the SPD and PS detectors have been  removed and the entire electronics of the system will be replaced. There will no longer be a hardware trigger and the aim is to process all the subdetectors at 40 MHz.
The electromagnetic  (ECAL) and hadronic (HCAL) calorimeters will remain in place. They are both based on a ``shashlik" technology of lead/iron and scintillators, and the light is collected by wave length shifting fibres~\cite{Amato:494264}. 
 The ECAL energy resolution is $10\% /\sqrt{E} \oplus 1\%$ where the energy is expressed in GeV. The information provided by this sub-detector is used as input to the particle identifications algorithms and flags photons, neutral pions or electrons. 
The HCAL energy resolution is significantly worse being $80\% /\sqrt{E} $,  however this was enough to provide information for the hardware trigger (L0) during Run 1 and 2. 

The new acquisition systems of both the ECAL and HCAL calorimeters will be driven by a control board (3CU).   The purpose of this board  is to  process and send critical information (the clock, the slow control signals and the fast and synchronous command) received through optical fibres from the main LHCb system to the front-end boards. A total of 23 control boards including spares are needed for both the electromagnetic and hadronic calorimeters.

 The LHCb operational master clock for data taking and the entire precise timing and synchronisation of the sub-detectors rely on the LHC bunch clock and the LHC orbit signal. The orbit signal marks each turn of the full LHC circulating bunch scheme (3563 steps). The readout supervisor system receives directly these two clocks from the RF-system of the LHC via an LHC Interface card located on the readout supervisor card. 
The LHC bunch clock is distributed to the front-end  and  readout boards with sufficiently low jitter (assumed for the moment to be ${\cal O}$(10 ps)), and constant and reproducible phase. 
To ensure this low jitter requirement, a great care was needed in the design of the clock tree distribution within the board. 
The readout supervisor card distributes the clock and the Fast Control commands to the readout board, and the interface readout board distribute the clock and the Fast Control command to the control board. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.35\linewidth]{figs/detector/calorimeters/Crate_Calo.pdf}
\caption{Schematic of a calorimeter crate.}
\label{fig:crate}
\end{figure}

The calorimeter crate mechanics are a standard 9U frame. They have two custom backplanes mounted in the back. The lower 3U backplane provides the power supplies, the Time Fast Control commands and the clock distribution. The upper 6U backplane is dedicated for the exchange of signals between the boards  inside the crate and with the other crates.
A calorimeter front-end crate contains up to 16 front-end boards  which perform the acquisition of the detector channels, and in the middle of the crate, a reserved slot for the control board.

The main role of the  control board is to receive the GBT (GigaBit Transceiver) frame through the optical link and to extract the information which is needed by the front end boards inside a same crate: the 40 MHz clock, the Time Fast Control (TFC) commands and  Experiment Control System (ECS). Figure~\ref{fig:3CU_picture} shows a picture of the control board (3CU). The various parts of the board are clearly identified. The board contains : 
  \begin{figure}[h]
\centering
\includegraphics[width=0.45\linewidth]{figs/detector/calorimeters/3CU.jpg}
\caption{3CU board.}
\label{fig:3CU_picture}
\end{figure}
\begin{itemize}
\item A Versatile Link Transceiver-Receiver (VTRx), for the reception and transmission to the SOL40 which an interface board that allows is to interface the fast and the slow control to the front-end boards.
\item	A radiation tolerant chip that can be used to implement multipurpose high speed (3.2-4.48 Gb/s user bandwidth) bidirectional optical links (GBTX).
\item	A GBT-SCA ASIC, part of the GBT chip-set, to distribute control and monitoring signals to the on-detector front-end electronics and perform monitoring operations of detector environmental parameters. 
\item	A Microsemi FPGA (IGLOO2 family) which is in charge of the processing on the 3CU.
\end{itemize}
Except for the commercial FPGA, the components listed above were designed at CERN and are shared across various sub-detectors in the LHCb upgrade. 
Following the clock and TFC command (or from left to right on the picture), first the 3CU receives the clock and the TFC command through the optical transmitter (VTRx) and decoding inside the GBTX.
After processing inside the FPGA, the board transmits through  the 3U backplane these signals to all the front-end boards inside the same crate. 

A challenging aspect  of the board was the design of the schematic for the PCB (Printer Circuit Board) especially around the GBTX component, where the density of extracted links is very high, about 300 out of the 400 of the GBTX pins. 

Two prototypes of these boards are currently available in the lab in Orsay and have been validated, the final production of the board has been submitted. 
%

The next steps will be to start testing the whole setup in a crate at CERN using the central acquisition system. 
Later, we will proceed to install and commission the electronics and ramp up for data taking. 
%\begin{figure}[h]\centering
%\includegraphics[width=0.40\textwidth]{figs/detector/calorimeters/nPVs_Kstee.pdf}
%\includegraphics[width=0.40\textwidth]{figs/detector/calorimeters/nTracks_Kstee.pdf}
%\caption{Number of reconstructed primary vertices (left) and number of reconstructed tracks for Upgrade (black) and 2016 (pink) simulations.}
%\label{fig:multiplicity}
%\end{figure}
%
%\begin{figure}[h]\centering
%\includegraphics[width=0.3\textwidth]{figs/detector/calorimeters/bmass_Kstee_nobrem.pdf}
%\includegraphics[width=0.3\textwidth]{figs/detector/calorimeters/bmass_Kstee_1brem.pdf}
%\includegraphics[width=0.3\textwidth]{figs/detector/calorimeters/bmass_Kstee_2brem.pdf}
%\caption{Invariant mass of $B^0\to K^*e^+e^-$ when no bremsstrahlung (left), one bremsstrahlung (middle) or two bremsstrahlung photons (right) were added. }
%\label{fig:Kstee}
%\end{figure}

\newpage




%
%
%
%\begin{table}[!htbp]
%  \centering
%      \resizebox{0.8\textwidth}{!}{
%        \begin{tabular}{|l|c|c|}
%        \toprule
%          \multirow{2}{*}{Track type } &\multicolumn{2}{c|}{\textit{Sample 1}} \\ \cline{2-3}
%                                       &\OldAlgo & \HybridAlgo  \\
%                                       & $\epsilon$ (\clonerate)            & $\epsilon$ (\clonerate)   \\  \midrule
%          \textit{hasT}                                 &(50.9 $\pm$ 0.1) (2.4) $\%$    &(65.7 $\pm$ 0.1) (0.0) $\%$  \\
%          \textit{long}                                 &(75.3 $\pm$ 0.1) (2.3) $\%$    &(90.3 $\pm$ 0.1) (0.0) $\%$   \\
%          \textit{long} $P>5$\gevc                      &(85.0 $\pm$ 0.1) (1.4) $\%$    &(93.1 $\pm$ 0.1) (0.0) $\%$  \\
%          \textit{long from B}                          &(81.8 $\pm$ 0.2) (1.7) $\%$    &(92.1 $\pm$ 0.1) (0.0) $\%$   \\
%          \textit{long from B} $P>5$\gevc               &(87.0 $\pm$ 0.2) (1.3) $\%$    &(93.6 $\pm$ 0.1) (0.0) $\%$   \\
%          \textit{long from B or D}                     &(80.6 $\pm$ 0.2) (1.8) $\%$    &(91.8 $\pm$ 0.1) (0.0) $\%$   \\
%          \textit{long from B or D} $P>5$\gevc          &(86.6 $\pm$ 0.1) (1.3) $\%$    &(93.4 $\pm$ 0.1) (0.0) $\%$   \\
%          \UT+\scifi \textit{strange}                   &(71.6 $\pm$ 0.1) (2.5) $\%$    &(89.7 $\pm$ 0.1) (0.0) $\%$   \\
%          \UT+\scifi \textit{strange} $P>5$\gevc        &(85.4 $\pm$ 0.2) (1.4) $\%$    &(93.3 $\pm$ 0.1) (0.0) $\%$   \\
%          no\velo+\UT+\scifi \textit{strange}           &(72.2 $\pm$ 0.2) (2.4) $\%$    &(89.1 $\pm$ 0.1) (0.0) $\%$   \\
%          no\velo+\UT+\scifi \textit{strange} $P>5$\gevc&(85.3 $\pm$ 0.2) (1.4) $\%$    &(93.1 $\pm$ 0.2) (0.0) $\%$   \\
%        \bottomrule \toprule
%          \ghostrate                                    &(23.1 $\pm$ 0.1) $\%$          &(9.4  $\pm$0.1) $\%$         \\
%          \ghostrate (evt.avg)                          &12.0 $\%$                    &       4.9  $\%$          \\ 
%        \bottomrule \toprule
%
%          \hitpurity                                    &99.0 $\%$                    &      99.6 $\%$            \\
%          \hitefficiency                                &96.0 $\%$                    &      97.82 $\%$           \\ 
%          \bottomrule
%        \end{tabular}}\caption{Tracking performances comparison between the \OldAlgo and the \HybridAlgo algorithms.}\label{tab:efficienciessample1}
%  \end{table}



%%%%% Sample 2 from Strange UT+T
%%\begin{figure}
%%\begin{center}
%%  \includegraphics[angle=90,origin=c]{figs/detector/tracking/LongFromBD_S3.pdf}%Sample3_TDRHybridNoReco_Long.pdf}
%%  \caption{\small \textit{Sample 3}: \treffs plot distributions for \textit{long} tracks. The efficiencies comparison between the \HybridAlgo (in blue) and the \OldAlgo (in red).}
%%  \label{fig:Sample3Efflong} 
%%\end{center}
%%\end{figure}




      %%\begin{figure}
%%\begin{center}

        %%\includegraphics[angle=90,origin=c]{figs/detector/tracking/Sample1_Ghosts.pdf}      
     %%   \caption{\small \textit{Sample 1}: \ghostrate comparison between the \HybridAlgo (in blue) and the \OldAlgo (in red). The plots %%show also all the reconstructed track distributions from the two algorithm versions. Note that the $P$, $P_{t}$, $\eta_{\mbox{track}}%%$ and $\phi$ distributions are determined using solely the \scifi segment information.}
    %%\label{fig:Sample1Ghost} 
%%\end{center}
 %% \end{figure}
%%%%Sample3 Tracking Efficiency long fromB or D
%\begin{table}[!htbp]
% \centering
%      \resizebox{0.8\textwidth}{!}{
%        \begin{tabular}{l|c|c}
%
%        \toprule 
%          \multirow{2}{*}{Track type } &\multicolumn{2}{c}{\textit{Sample 3}}  \\ \cline{2-3}
%                                       &\OldAlgo    & \HybridAlgo                           \\
%                                                    & $\epsilon$ (\clonerate) & $\epsilon$ (\clonerate)   \\ \midrule
%          \textit{hasT}                             &(53.4 $\pm$ 0.1)(2.8) $\%$ & (67.2 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long}                             &(77.1 $\pm$ 0.1)(2.6) $\%$ & (90.6 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long} $P>5$\gevc                  &(88.2 $\pm$ 0.1)(1.8) $\%$ & (94.8 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long from B}                      &(84.4 $\pm$ 0.1)(2.0) $\%$ & (93.4 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long from B} $P>5$\gevc           &(90.0 $\pm$ 0.1)(1.6) $\%$ & (95.4 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long from B or D}                 &(83.3 $\pm$ 0.1)(2.2) $\%$ & (92.9 $\pm$ 0.1)(0.0) $\%$\\
%          \textit{long from B or D} $P>5$\gevc      &(89.8 $\pm$ 0.1)(1.6) $\%$ & (95.3 $\pm$ 0.1)(0.0) $\%$\\
%          \UT+\scifi \textit{strange}               &(73.6 $\pm$ 0.1)(3.0) $\%$ & (89.7 $\pm$ 0.1)(0.0) $\%$\\
%          \UT+\scifi \textit{strange} $P>5$\gevc    &(88.7 $\pm$ 0.2)(1.8) $\%$ & (95.2 $\pm$ 0.1)(0.0) $\%$\\
%          no\velo+\UT+\scifi \textit{strange}       &(74.2 $\pm$ 0.2)(2.8) $\%$ & (89.4 $\pm$ 0.1)(0.0) $\%$\\
%          no\velo+\UT+\scifi \textit{strange} $P>5$\gevc &(88.6 $\pm$ 0.4)(1.7) $\%$ & (95.0 $\pm$ 0.1)(0.0) $\%$ \\ 
%          \bottomrule \toprule
%          \ghostrate                                & (21.3 $\pm$ ) $\%$   & (7.9  $\pm$ 0.1)     $\%$     \\
%          \ghostrate (evt.avg)                      & 10.9 $\%$               &  4.5 $\%$              \\ 
%          \bottomrule \toprule
%          \hitpurity                                & 99.1 $\%$               &  99.7 $\%$             \\
%          \hitefficiency                            & 94.9 $\%$               &  96.8 $\%$        \\
%          \bottomrule    
%        \end{tabular}}\caption{Tracking performances comparison between the \OldAlgo and the \HybridAlgo algorithms for \textit{Sample 3}.}\label{tab:efficienciessample3}
%  \end{table}%

  


==> experimentally.tex <==
% !TEX root = thesis.tex
\chapter{Allegro}





\epigraph{\textit {"Once you kill a cow,\\ you gotta make a burger"}}{Lady Gaga}

\section {Dear \bquark-baryons}
The  first observed baryon with a \bquark-quark was the \Lb baryon ($bud$). This isospin-zero particle was discovered in \jpsi \Lz decays, at the UA1 detector in proton-antiproton collisions at CERN~\cite{Albajar:1991sq} and was later confirmed and studied by several experiments. 
\Lb particles are produced abundantly in the proton-proton collisions of the LHC,  their production rate\footnote {In 13 TeV proton-proton collisions.} relative to $B$-mesons is $f_\Lb/ (f_u + f_d) = 0.259~\pm~0.018$~\cite{Aaij:2019pqz}. 


 \begin{figure}[h!]
\centering
\includegraphics[scale=0.35]{figs/Lb-5pb.png}
\caption{Most probably one of the first \Lb distributions seen at LHCb.}
\label{fig:Lb-5pb}
\end{figure}
%%

Figure~\ref{fig:Lb-5pb} shows the \jpsi \Lz invariant mass using 5 pb$^{-1}$ from the 2010 dataset, when a requirement on the decay time of the \Lb candidate to be higher than 0.3 ps is applied. I am particularly fond of this plot, because  it was one of the first distribution of \Lb decays  seen at LHCb and it  really marked the start of my research activities with \bquark-baryons. With more data, more \bquark-baryons were seen and discovered, in particular I was involved in the studies of the \Xibm and \Omegab baryons at LHCb. 
 For what concerns NP searches, \bquark-baryons allow to verify the anomalies in a different hadronic environment.  Furthermore, since they carry half-integer spin, NP-sensitive observables which are not present in $B$-mesons can be measured in \Lb decays. Table~\ref{tab:bbaryons} summarises the current experimental knowledge on the lightest \bquark-baryons.

\begin{table}[h]
  \centering
  \caption{Properties of the lightest \bquark-baryon states. Based on Ref.~\cite{PDG}.}
  \label{tab:bbaryons}
  \begin{tabular}{|c|c|c|c|c|c|r|}%P{75mm}

\hline
Name & \makecell{Quark\\content} & Mass, \mevcc & \makecell{Lifetime\\or width} & $J^P$ & ($I$,$I_3$) & $S$ \\
\hline
\Lb & $udb$ & $5619.60 \pm 0.17$ & $1.470 \pm 0.010$ ps & $1/2^+$ & $(0,0)$ & $0$\\
\hline
\Xibz & $usb$ & $5791.9 \pm 0.5$ & $1.479 \pm 0.031$ ps & $1/2^+$ & $(1/2,1/2)$ & $-1$\\
\hline
\Xibm & $dsb$ & $5797.0 \pm 0.9$ & $1.571 \pm 0.040$ ps & $1/2^+$ & $(1/2,-1/2)$ & $-1$\\
\hline
$\Sigmares^+_{\bquark}$ & $uub$ & $5810.55 \pm 0.25$ & $4.83\pm0.48$ \mevcc & $1/2^+$ & $(1,1)$ & $0$\\
\hline
$\Sigmares^0_{\bquark}$ & $udb$ & \multicolumn{2}{c|}{not yet observed} & $1/2^+$ & $(1,0)$ & $0$\\
\hline
$\Sigmares^-_{\bquark}$ & $ddb$ & $5815.64 \pm 0.28$ & $5.33\pm0.56$ \mevcc & $1/2^+$ & $(1,-1)$ & $0$\\
\hline
$\Xires'^0_\bquark$ & $usb$ & \multicolumn{2}{c|}{not yet observed} & $1/2^+$& $(1/2,1/2)$ & $-1$\\
\hline
$\Xires'^-_\bquark$ & $dsb$ & $5935.02 \pm 0.05$ & $<0.08$ \mevcc & $1/2^+$ & $(1/2,-1/2)$ & $-1$\\
\hline
\Omegab & $ssb$ & $6046.1 \pm 1.7$ & $1.64\pm0.18$ ps & $1/2^+$ & $(0,0)$ & $-2$\\
\hline
\hline
$\Sigmares^{*+}_{\bquark}$ & $uub$ & $5830.28 \pm 0.28$ & $9.34\pm0.54$ \mevcc & $3/2^+$ & $(1,1)$ & $0$\\
\hline
$\Sigmares^{*0}_{\bquark}$ & $udb$ & \multicolumn{2}{c|}{not yet observed} & $3/2^+$ & $(1,0)$ & $0$\\
\hline
$\Sigmares^{*-}_{\bquark}$ & $ddb$ & $5834.73 \pm 0.30 $ & $10.68\pm0.68$ \mevcc & $3/2^+$ & $(1,-1)$ & $0$\\
\hline
$\Xires^{*0}_\bquark$ & $usb$ & $5949.8\pm1.4$ & $0.90\pm0.18$ \mevcc & $3/2^+$& $(1/2,1/2)$ & $-1$\\
\hline
$\Xires^{*-}_\bquark$ & $dsb$ & $5955.33 \pm 0.13$ & $1.65\pm0.33$ \mevcc & $3/2^+$ & $(1/2,-1/2)$ & $-1$\\
\hline
$\Omegares^{*-}_\bquark$ & $ssb$ & \multicolumn{2}{c|}{not yet observed} & $3/2^+$ & $(0,0)$ & $-2$\\
\hline

 \end{tabular}
\end{table}



\section{Mass measurements}
\label{sec:mass-exp}
My main collaborators for the measurements~\cite{Aaij:2013qja}  discussed in this section were Sneha Malde  and Matthew Needham. 
Within the SM of particle physics, mesons and baryons are colourless objects composed of quarks and gluons as discussed in Chapter 1. These systems are bound through the strong interaction,
described by QCD. A basic property of hadrons that can be compared to QCD theoretical predictions is their masses.
In 2008,  there was the controversial discovery of the \myOb first claimed by the D\O~experiment with $ M(\myOb)= 6165\pm10(\textrm{stat}) \pm 13(\textrm{syst})$ \mevcc. A few months later the CDF collaboration also reported a measurement of the mass of this baryon    $ M(\myOb)= 6054.4\pm6.8(\textrm{stat})\pm 0.9(\textrm{syst}) \mevcc$. Assuming the uncertainties to be uncorrelated across experiments, the difference between these two measurements, $111 \pm 12 (\textrm{stat}) \pm 13 (\textrm{syst}) \mevcc$, represents a discrepancy of more than six standard deviations. 
What was particularly puzzling about the D\O~measurement is that it was in disagreement with the expectations of mass splittings inferred from quark model predictions of both beauty and charm particles.   For example, as shown in Chapter 1,  the theoretical predictions for the \myOb mass are fairly broad, they lie in the range of 5940 - 6120 \mevcc. 

%\paragraph{Momentum scale}
%%
%%
A key aspect of mass measurements is controlling the momentum scale of the experiment. A time-dependent momentum scale calibration procedure  was used to ``correct" the measured \bquark-baryon masses~\cite{Karliner:2008sv}. 

%%
%%
\begin{figure}[h!]
\centering
\includegraphics[scale=0.28]{figs/masses/m-and-sigma-jpsi.png}
\caption{ Measured $\jpsi \to \mumu$ mass (top) and resolution (bottom) as a function of
run number during the entire 2010 data-taking period. The steps (indicated with vertical
lines) correspond to the times when the TT operating temperature was altered.}
\label{fig:trends}
\end{figure}
%%
%%

The principles behind the momentum scale calibration can be described as follows. For a two-body decay $P\to c_1c_2$ relativistic mechanics gives: 
\begin{equation}
m_{12}^{2} = (E_1+E_2)^2 - (\vec{p}_1 + \vec{p}_2).  (\vec{p}_1 + \vec{p}_2).
\end{equation}
%%
%%
%Let $1-\alpha$ be the factor by which each track vector momenta of the final state particles need to be multiplied in order to obtain the true mass $m_P$ of the decaying particle.  
It can be shown that if the momentum scale is wrong by a factor (1-$\alpha$), the the measured mass $m_{12}$ is given to first order in $m/p$ by:
\begin{equation}
m_{12} = \frac{m_P^2 - f}{(1-\alpha)^2} + f, 
\end{equation}
where
\begin{equation}
f = m_1^2 + m_2^2 + \frac{p_2}{p_1}m_1^{2} +  \frac{p_1}{p_2}m_2^{2}.
\end{equation}
If $\alpha \ll 1$ this expression simplifies, to first order, to  
%%
\begin{equation}
\Delta m = \alpha \frac{f- m_P^2}{m_P}
\end{equation}
where $\Delta m= m_P - m_{12}$.  
For decays of quarkonia or heavy hadrons where the mass of the final state particles can be neglected with respect to the parent particle, the correction needed can be written as: 
\begin{equation}
\Delta m = -\alpha ~ m_P. 
\end{equation}
%\newpage

A set of two-body decay modes was considered for the calibration of the momentum scale.  The central value of the momentum scale is taken as the value of $\alpha$ extracted using $\jpsi\to \mu^{+} \mu^{-}$ decays. An example of the trends is shown in Figure:~\ref{fig:trends}.



\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth] {figs/masses/alpha17New.pdf}
\caption{\small Average momentum scale bias $\alpha$ extracted from the
reconstructed mass of various decay modes after the momentum calibration procedure.
The $\KS$ decays are divided into two categories: those where the two child tracks have hits in the vertex detector (labelled L)
and those without (labelled D). The black error bars represent the statistical uncertainty whilst the (yellow) filled areas also include contributions
to the systematic uncertainty from the fitting procedure, the effect of QED radiative corrections, and the uncertainty
on the mass of the decaying meson~\cite{PDG}.
The (red) dashed line shows the assigned uncertainty of $\pm 0.03\%$ on the momentum scale.}
\label{fig:scale}
\end{figure}

 To understand the odd  behaviour in the trends (around Run 500), we relied on the  log-books of the LHCb data shifter. We identified that it was due to a  temperature variation of the  TT tracker.  To evaluate the impact of these variations, two versions of the detector alignment  were tested, the standard one and  one were the hits from the TT are systematically excluded from the track reconstruction. 
 The whole exercise (track reconstruction, selection, mass fits) was repeated. 
 Finally, the impact of the TT temperature variation was found not to be significant on the observables of interest, and no additional systematic uncertainty was assigned. 

 The systematic uncertainty on the momentum scale was taken as the difference between the values of $\alpha$ extracted form $\jpsi\to \mu^{+} \mu^{-}$  and $\KS\to \pi^{+} \pi^{-}$ decays. The calibration was cross-checked using other \bquark-decay modes.

 
Figure~\ref{fig:scale} shows a summary of the momentum scale calibration. To measure the impact of systematic effects, the overall momentum scale was shifted by $\alpha = 0.5 \times10^{-3}$  with little  variation amongst the modes. The  momenta of all the tracks used to form the \bquark-baryon candidates are multiplied by $1-\alpha$ before  any mass constraint is applied, the uncertainty on the knowledge of $\alpha$ is later propagated to the final measurement as a systematic uncertainty on the mass measurements. 
%----
%----
%\paragraph{Extraction of the observables}

The decay modes employed to measure the masses of the \Lb, \Xibm and \Omegab, were $\jpsi \Lz$, $\jpsi \Xi(\to \Lz \pi^-)$  and $\jpsi \Omega (\to\Lz \kaon^-)$ respectively. The \Lz particle that decays to a pion and a proton travels a relatively long distance in the LHCb detector, $\cal O$(cm).  The child tracks from the \Lz baryon are referred to as long tracks if they leave energy deposits in the vertex locator or downstream tracks if they don't.  To improve the resolution on the measured mass of the \bquark-baryons by almost a factor two, a constraint on the known masses of the \jpsi and the \Lz particles was systematically applied.

For these measurements simple cut-based selections relying on the kinematic properties of the final state particles and their identification probabilities were sufficient to select clean signal samples. The values of the masses were extracted from  maximum likelihood fits to the invariant mass. The fit model was based on a Gaussian function to describe the signal and an exponential  function to describe the combinatorial background. In the case of the \Omegab baryon, given the discrepancy which was observed between the previous measurements, the fitted value of the mass was kept blind throughout the analysis process, although not the mass distribution itself.  The results are reported in Table \ref{tab:average}. 
\begin{table}[t]
\caption{\small Comparison of the $b$-baryon mass measurements using the full LHCb 2011 data sample with
the single most precise results from the ATLAS~\cite{Aad:2012shb}, CDF~\cite{Aaltonen:2009ny,Acosta:2005mq}
and \dzero~\cite{Abazov:2008qm,Abazov:2007am} collaborations, and with the PDG averages~\cite{PDG2012}.
The PDG averages (2014) contain the results from CDF and D\O~ as well as the \myLb measurement from LHCb performed with the 2010 data sample.
The quoted errors include statistical and systematic uncertainties. All values are in\,\mevcc.}
\vspace{1.5ex}
\centering
\begin{tabular}{l|l|l|l}
            &  \multicolumn{1}{c|}{$M(\myLb)$}
            &  \multicolumn{1}{c|}{$M(\myXb)$}
            &  \multicolumn{1}{c }{$M(\myOb)$} \\ 
       \hline
      ATLAS &  $5619.7 \pm 1.3~$ & --                & --                \\
       CDF  &  $5619.7 \pm 1.7~$ & $5790.9  \pm 2.7$ & $6054.4  \pm 6.9$ \\ 
     D\O  &  --                & $5774~~\,\pm 19 $ & $6165~~\,\pm 16$  \\ 
       PDG (2014) &  $5619.4 \pm 0.7~$ & $5791.1  \pm 2.2$ & $6071~~\,\pm 40$  \\ 
\hline
       LHCb &  $5619.5 \pm 0.5~$ & $5795.8  \pm 1.0$ & $6046.0  \pm 2.3$ \\ 
\end{tabular}
\label{tab:average}
\end{table}
%----
%----

To take into account the ``look elsewhere effect'', the significance of the \myOb signal was determined using a large  number of pseudo-experiments with background only. For each pseudo-experiment a  sample of mass values with the same size as the data sample  is generated using the exponential background distribution determined from the fit to the data candidates. 
We determined the probability that, in these pseudo-experiments, any signal  seen in the mass range 5.8--6.3\gevcc would lead to a value of $\ln({\cal L}_{\rm max}/{\cal L}_0)$ 
larger than in the data,  and interpret it as the probability that the observed \myOb peak in
the data is due to a statistical fluctuation of the background.  The distribution of $\ln({\cal L}_{\rm max}/{\cal L}_0)$, determined with 
2,500,000 pseudo-experiments, is shown in Figure~\ref{fig:dll}. The fact that no pseudo-experiment yields a 
value larger than the data suggests a $p$-value smaller than 4$\times 10^{-7}$, which translates to a statistical significance consistent with $6.8\,\sigma$.

The LHCb collaboration measured the  \myOb mass, using the hadronic final state \Omegac (\to \proton\kaon \kaon \pion )\pion \cite{Aaij:2016dls}. The result was found to be in agreement with the measurement discussed in this section and the result from CDF. 
The measurement from the D\O~ experiment is no longer taken into account in the PDG averages~\cite{PDG}. 
Spectroscopy and mass measurements have a bright future at LHCb, the first observation of \myOb baryon  excited states  was reported recently in Ref.~\cite{Aaij:2020cex}.
\begin{figure}[t]
\centering
\includegraphics [width=0.50\textwidth] {figs/masses/Omega_significance.pdf}
\caption{\small Distribution of the negative log-likelihood difference $\ln({\cal L}_{\rm max}/{\cal L}_0)$ in $2.5\times 10^{6}$ pseudo-experiments with background only. The red arrow corresponds to the value observed in the data.}
\label{fig:dll}
\end{figure}


\section{Lifetime measurements}
My main collaborators on the lifetime measurements~\cite{Aaij:2014owa} were Francesca Dordei and Greig Cowan. Lifetime measurements  are often considered to be  the ``bread \& butter" of a flavour experiment.  Whoever thinks this should be sent to jail.  The analysis discussed in this section grouped many $b$-hadrons.  The decays of these hadrons all shared   $J/\psi X$ topologies  displayed in Figure~\ref{fig:sketch}, where $X$ was  required to be $\kaon^{+}, \KS, \Kstarz, \phi$ or a  \Lz.   
%%%
\begin{figure}[h!]
\centering
\includegraphics[scale=0.35]{figs/lifetimes/bdecay.png}
\caption{Sketch of the decay of a $b$-hadron to  a  $J/\psi$ and an additional particle X. The $b$-hadron is produced at
the primary vertex (PV) and it decays at the decay vertex (SV). The length $L$ is the spatial
separation between the two vertices.}
\label{fig:sketch}
\end{figure}
%%%%
Thanks to the clean dimuon signatures of these decays and the usage of mass constraints on the known values mass of  the \jpsi, \KS and \Lz particles,  simple cut-based selections were found to be sufficient to select all the signals. 
Furthermore, cut-based selections were even favoured to more sophisticated multivariate ones, since we were trying to track down all the possible sources of biases that might influence the measured lifetimes. 
The decay time, $t$, of a particle in its rest frame, can be computed as follows: 
\begin{equation}
t = L ~\frac{m}{|\,\vec{p}\,|}
\end{equation}
where $L$ is the flight distance travelled by the \bquark-hadron, $p$ is the reconstructed three-momentum and $m$ its reconstructed mass. 

Two approaches were used to access the observable of interest. The first one was based on a two-dimensional likelihood fit to the invariant mass and decay time of the \bquark-hadron. In the second approach, $_{s}\cal{W}$eights~\cite{Pivk:2004ty} were extracted from a fit to the invariant mass distribution and exploited to subtract the background components from the lifetime distributions, which were then fitted.  While doing the analysis it was thought  to be very useful to have two methods for cross-checks. 


The signal probability density function used in the lifetime fit  to extract the observable of interest $\tau_{H_{b}}$ can be written as follows: 
\begin{equation}
[e^{(t ^\prime/\tau_{H_{b}})} \otimes {\cal R} (t, t^\prime)] \times  \textrm {Acc} (t)
\end{equation}
A sketch of a typical shape of the decay time resolution ($\cal {R}$) and the decay time acceptance (Acc) are shown in Figure~\ref{fig:acceptances}.
Given that the expected statistical uncertainty for these measurements was around a few femtoseconds, it was mandatory to have a very good control of the acceptance effects in particular. 
The decay-time resolution was measured using  data. At the start of the LHCb data taking,  large samples of  ``prompt-$J/\psi$" decays were recorded with dedicated trigger lines. Given that they were produced at zero lifetime, the width of their decay time distribution was dominated by the decay time resolution. Typical values of the decay time resolution for these decay modes was about 50 fs. 
\begin{figure}
\centering
\includegraphics[scale=0.40]{figs/lifetimes/sketch_acceptance.png}
\caption{Sketch of a decay-time distribution, decay-time resolution and decay-time acceptance of a \bquark-hadron ($x$-axes not to scale). }
\label{fig:acceptances}
\end{figure}

Understanding the decay-time acceptances turned out to be a tricky job.  Figure~\ref{fig:LbAnatomy} displays the breakdown of all the effects entering the decay-time acceptance seen in \Lb decays. When we first started to test the fitting procedure using simulated samples, on which the full reconstruction and event selection was applied, biases up to 18 fs were observed for the decay modes where all the tracks were decaying inside the vertex locator. The biases were smaller $\sim$10 fs for decays with long-lived particles (\KS and \Lz). 
This observation allowed to point towards effects coming from the vertex locator  reconstruction. 
And indeed, an assumption that the tracks were produced in a  region close to the interaction region was used in the pattern recognition algorithms.  This assumption was the main cause for the ``upper lifetime" acceptance. 
Since this was the start of LHCb data taking and the time-dependent analyses did not have the maturity that they have now, we did not feel comfortable  to simply plug whatever bias was measured from simulation into the data fit.  We developed a data-driven method to address this point. A large sample of \BuToJPsiK decays was used where the kaon was reconstructed without using the information from the vertex locator\footnote{The \kaon was reconstructed using only the downstream tracking.}.
For the purpose of these studies, we reprocessed both the data and simulation samples using the downstream tracking on the kaon.  The vertex locator reconstruction  efficiency was then computed using a tag-and-probe technique. 

A parametrisation based on the distance of closest approach of one of the final state particles allowed to model the efficiency of this algorithm on data. This parametrisation took into account the different tunings of the reconstruction in the trigger and offline, as well as correlations between tracks. Weights were extracted from the vertex locator reconstruction efficiency distribution and applied to the signal candidates in data to correct for this effect. 

The remaining effects that contributed to the decay time acceptances were: the position of the primary vertex, the vertex quality of the fit which was worse for tracks with a small opening angle (for example $\phi\to\Kp\Km$), a requirement on the displacement of the \jpsi from the primary vertex in the software trigger and in the stripping selection. 

\begin{figure}
\centering
\includegraphics[scale=0.450]{figs/lifetimes/Lb_anatomy.png}
\caption{\Lb acceptance steps as a function of the different reconstruction, selection and trigger requirements in the analysis.}
\label{fig:LbAnatomy}
\end{figure}
The absolute lifetimes of the $b$-hadrons are reported in Table \ref{tab:sfit_fit_results}. Besides the \Lb measurement all the others were the world's best measurements. 

% 
The early  measurements of the ratio of \Lb to \Bz lifetimes  were mainly driven by the Tevatron, and gave results  which were considerably smaller than the theoretical expectation~\cite{Ito:1997qq, Gabbiani:2004tp,Altarelli:1996gt}. It was considered for a while by the theory community that additional operators should be included in the description of the \Lb amplitude to account for these differences. 
However, today the combined measurement of the \Lb lifetime from LHCb,  $1.468 \pm 0.009 \pm 0.008$ ps is in agreement with most of the predictions from HQET~\cite{Lenz:2015dra}.  With work, it is fair to say that we closed the \Lb lifetime saga.
\begin{table}[h]
\caption{\small Fit results for the \Bu, \Bd, \Bs mesons and $\Lb$ baryon lifetimes. The first uncertainty is
statistical and the second is systematic.}
\centerline{
\begin{tabular}{lc}
	Lifetime		&	Value [\ps]\\
	\hline
	$\tau_{\BuToJPsiK}$	  &	1.637 $\pm$ 0.004 $\pm$ 0.003 \\
	$\tau_{\BdToJPsiKst}$&	1.524 $\pm$ 0.006 $\pm$ 0.004 \\
	$\tau_{\BdToJPsiKS}	$&	1.499 $\pm$ 0.013 $\pm$ 0.005 \\
	$\tau_{\LbToJPsiL}$	  &	1.415 $\pm$ 0.027 $\pm$ 0.006 \\
	$\tau_{\BsToJPsiPhi}	$&	1.480 $\pm$ 0.011 $\pm$ 0.005 \\
	\hline
\end{tabular}
}
\label{tab:sfit_fit_results}
\end{table}



The cherry on the cake  from this analysis, was that the  lifetimes of \mbox{\BdToJPsiKst} and \BdToJPsiKS decays were used to
measure $\Delta\Gamma_d/\Gamma_d$ as suggested in Ref.~\cite{Gershon:2010wx}.
Flavour-specific final states such as \BdToJPsiKst have
\mbox{$\mathcal{A}_{\Delta \Gamma_d}^{\BdToJPsiKst}=0$}, while $\mathcal{A}_{\Delta \Gamma_d}^{\BdToJPsiKS} = \cos (2\beta)$ to a good approximation in the SM,  where for a given final state $f$:
\begin{equation}
\mathcal{A}_{\Delta \Gamma_d}^{f}= \frac{2 \textrm{Re} (\lambda_f)}{1+ |\lambda_f|^2}, \mbox{ ~and~ } \lambda_f = \frac{q}{p}\frac{\bar{A}_f}{A_f} 
\end{equation}
where, 
parameters ${\bar{A}_f}$ and ${A_f}$ are the complex amplitudes for the decay of a  $\bar{\Bd}$ and \Bd   to the final state $f$, respectively,
and 
 \mbox{$\beta \equiv \arg\left[-(V_{cd}V^*_{cb})/(V_{td}V^*_{tb})\right]$} is one of the CKM unitarity triangle angles~\cite{Amhis:2019ckw}.
Hence, the two effective lifetimes can be expressed as
\begin{alignat}{2}
\label{eqn:Bd_eff_Kst}
\tau_{\Bd \rightarrow J/\psi K^{*0}} &= \frac{1}{\Gamma_d}\frac{1}{1-y_d^2} \left( 1+ y_d^2 \right),\\
\label{eqn:Bd_eff_KS}
\tau_{\Bd \rightarrow J/\psi K^0_S} &= \frac{1}{\Gamma_d}\frac{1}{1-y_d^2} \left( \frac{1+2 \cos(2\beta) y_d + y_d^2}{1+\cos(2\beta) y_d} \right).
\end{alignat}
Using the effective lifetimes reported in Table~\ref{tab:sfit_fit_results} and
$\beta = (21.5^{+0.8}_{-0.7})^{\circ}$~\cite{Amhis:2019ckw},
a fit of $\Delta\Gamma_d$ and $\Gamma_d$ to the expressions in
Eq.~(\ref{eqn:Bd_eff_Kst}) and Eq.~(\ref{eqn:Bd_eff_KS}) leads to
\begin{align} 
\Gamma_d &= \phantom{+}0.656 \pm 0.003  \pm 0.002\invps ,\\
\Delta \Gamma_d &= -0.029 \pm 0.016 \pm 0.007\invps ,
\end{align}
where the first uncertainty is statistical and the second is systematic. 
The correlation coefficient between $\Delta\Gamma_d$ and $\Gamma_d$ 
is $0.43$ when including statistical and systematic uncertainties.
The combination gives
\begin{equation}
\frac{\Delta \Gamma_d}{\Gamma_d} = -0.044 \pm 0.025  \pm 0.011,
\end{equation}
consistent with the SM expectation: $40.9^{+8.9}_{-9.9}\times 10^{-4}$~\cite{Lenz:2006hd,Lenz:2011ti} and the current world-average value~\cite{Amhis:2019ckw}.





\section{Lepton universality test}
In this section,  I will discuss the first test of lepton universality measurement with \bquark-baryons from Ref.\cite{Aaij:2019bzx}. This measurement was  the PhD thesis of Vitalii Lisovskyi~\cite{Lisovskyi:2699822} whom I  co-supervised together with Marie-H\'el\`ene.  We were then joined by Carla Marin Benito who is funded by the ANR {\tt BACH} project. 

In the SM the couplings of the $W$ and $Z$ bosons to all charged lepton species are identical and a
large number of experiments where the electroweak bosons are directly produced have
tested this property. The  LEP measurements of the $Z\to \epem$, $Z\to\mu^{+}\mu^{-}$ and $Z\to\tau^+\tau^-$ partial widths  are in very good agreement with each other~\cite{ALEPH:2005ab}: 
\begin{equation}
\frac{\Gamma (Z \to \mu^{+}\mu^{-} )}{\Gamma ( Z \to \epem) } =  1.0009 \pm 0.0028. 
\end{equation}
\begin{equation}
\frac{\Gamma (Z \to \tau^{+} \tau^{-}) }{\Gamma (Z \to \epem)}  = 1.0019\pm  0.0032.
\end{equation}
In addition to the measurement at the $Z$ pole, a good agreement was also found in the LHC measurements~\cite{Aaboud:2016btc}. A detailed review of further LU tests with $W$ bosons, as well as in  light pseudo scalar mesons can be found in Ref.~\cite{Bifani:2018zmi}.
Under the assumption of LU, all the decay widths of the $Z$ boson decay to leptons  are expected to be equal in the SM. 
%As mentioned in Chapter 1, LU was tested by the LHCb collaboration and $B$-factories using both \Bu and \Bz decays.  


As it was shown in the previous sections, \Lz particles have a rather long lifetime and a lower reconstruction efficiency in comparison to particles produced close to the interaction point. Therefore, the overall yields of $\Lb \to \Lz\ell^{+}\ell^{-}$ decays were expected to be smaller than \LbTopKll decays. This is what motivated the choice of this particular decay for the LU test. 
Table~\ref{tab:state_Lb} summarised the current experimental knowledge on  \Lb baryon to $pKX$ final states. What can be seen is that at the time when this analysis started only the branching fraction of the decays to charmonia  decays were known.   The $pK$ resonant structure was resolved only for the \jpsi mode\footnote{This analysis that led to the discovery of the states compatible with pentaquark particles.
}, as shown in Figure~\ref{fig:pKmm_2016_059}. 

\begin{table}[ht!]
  \centering
  \caption{Status of the decay modes of interest of the \Lb baryon before the work discussed in this section.}
  \label{tab:state_Lb}
  \begin{tabular}{l|c|c|c|c}
    \toprule
%   \hline
    Decay mode & Observed &  Published &  BR measured &  Refs.\\
\hline
%    \midrule
    \LbTopKmm & Yes & Yes & No & \cite{LHCb-PAPER-2016-059} \\
    \LbTopKee & No & No & No &  N/A \\
    \LbTopKJPsi & Yes & Yes & $(3.17\pm0.04^{+0.57}_{-0.45})\times10^{-4}$ & \cite{LHCb-PAPER-2015-032} \\
    \LbTopKPsi & Yes & Yes & $(6.6^{+1.2}_{-1.0})\times10^{-5}$ & \cite{LHCb-PAPER-2015-060} \\
    \LbTopKG & (Yes) & No & No & N/A\\
\hline
%    \bottomrule
 \end{tabular}
\end{table}

\begin{figure}[thb!]
    \centering
        \begin{subfigure}[t]{0.40\textwidth}
        \centering
        %\raggedleft
        \includegraphics[height=2.5in]{figs/lu/mkp-default.pdf}
      \end{subfigure}%
        \begin{subfigure}[t]{0.40\textwidth}
        \centering
        %\raggedleft
        \includegraphics[height=2.3in]{figs/lu/pKmm_2016_059.pdf}
    \end{subfigure}%
    
        
    \caption{Invariant mass of $m(pK)$ in \LbTopKJPsi (left) and \LbTopKmm (right) data. Figures taken from and Ref.~\cite{LHCb-PAPER-2015-029} Ref.~\cite{LHCb-PAPER-2016-059} respectively.}
    \label{fig:pKmm_2016_059}
\end{figure}


The identification of electrons is peculiar with respect to the other charged  tracks in the LHCb detector.  Electrons\footnote{The average transverse momentum of electrons from $b$-decays is a couple of GeV. } emit bremsstrahlung radiation when they interact with the material in the detector. 
This radiation is emitted colinearly to the electron direction. This effect will have an impact on the electron momentum estimate. 
If the bremsstrahlung photon is emitted before the magnet, it will continue its path in the original direction of the electron, while the electron will be bent in the magnet. Hence the electron and the photon will not be absorbed in the same cells of the electromagnetic calorimeter. 
The measured momentum of the electron is lower given that it lost some of its energy to the photon. 
In this configuration the emitted bremsstrahlung does not affect the measured ratio $E/p$ used in the electron identification. 
If on the other hand the photon is emitted after the magnet, but before the electromagnetic calorimeter, the momentum of the electron has already been estimated. The photon and the electron end up in the same cell. Hence their combined energy release provides the original electron energy and here also  $E/p$ is not affected. 

In order to account for the bremsstrahlung effects, dedicated algorithms are used inside the LHCb reconstruction algorithms to correct for them.  One of the main impacts of the bremsstrahlung radiation is the very striking and non-trivial shape of the $b$-hadron invariant mass distribution. Typically, three\footnote{One per bremsstrahlung category.} bifurcated Crystal-Ball functions are necessary to describe the shapes decays involving electrons like \BuToKee, \BdToKstee or \LbTopKee. Furthermore, because of the worse overall mass  resolution with respect to muon modes, great care is needed to model the partially reconstructed backgrounds which populate the left hand side of the invariant mass distributions. 
These distributions were quite a change of scenery to me, given that I was used to very clean dimuon signatures. 
%
%
 \begin{figure}[h!]
    \centering
    \includegraphics[scale=0.5]{figs/detector/calorimeters/ebrem.png}
    \caption{Illustration of the bremsstrahlung photons emitted by an electron before and after the magnet.}
    \label{fig:brem}
\end{figure}
%
%
The observable of interest  \invRpK  can be written as:
\begin{equation}
 \invRpK = \frac{BR(\LbTopKee)}{BR(\LbTopKmm)} \times \frac{BR(\LbTopKJPsimm)}{BR(\LbTopKJPsiee)}.
\end{equation}
It is defined this way to ensure the best possible cancellation of  effects that can be introduced by the differences in the treatment of reconstruction effects between muons and electrons. For example, the universality of the \jpsi decays which has been already tested very precisely: 
%
%
%
\begin{equation}
    \frac{\Gamma_{\jpsi\to\epem}}{\Gamma_{\jpsi\to\mumu}}=1.0016\pm0.0031,
\end{equation}
is used to evaluate \invRpK as a double ratio rather than a more obvious single ratio.

One of the most frequent questions that the proponents of the analysis and myself received since the publication of our results is: ``Why did you measure \invRpK and not \RpK ?".
The answer to this question is  illustrated in Figure \ref{fig:simfit_RpK=1_NLL} which indicates better behaviour of the log-likelihood profile for \invRpK with respect to \RpK. 
This effect is driven by the fact that a log-likelihood profile will be more Gaussian if the smaller number (the electron yield in our case) is at the numerator rather than the denominator. 
The first \RK and \RKst measurements were done at the $B$-factories where the overall yields of the electron and muon rare modes were of about the same size and this particular point was not as relevant for them.


The \invRpK analysis was performed in trigger categories. Indeed it was shown that the kinematics of the decay vary depending on whether the candidates were triggered by the hardware trigger based on the electromagnetic calorimeter or by the ``other" particles in the event. 
In the jargon of LHCb, this classification is called TIS for Triggered Independently of the Signal and this was the prime category for the electron channel, or TOS for Trigger On Signal and this was the second category. In our construction these two categories were exclusive. 
For decays involving muons in the final state, only one trigger category based on the information from the muon stations in the hardware level was used.


To reduce the combinatorial background,  multivariate approaches  based on boosted-decision trees were employed. The algorithms were trained on simulated signal samples which were reweighed to account for differences between data and simulation.  The background samples were obtained from the upper side bands of the invariant mass data distribution and $k$-folding was used to  avoid biases in the training phase. 



\begin{figure}[htbp!]
    \centering
   \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.9in]{figs/lu/nll_RpK.pdf}
    \end{subfigure}%
      \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[height=1.9in]{figs/lu/nll_RpK_inv.pdf}
    \end{subfigure}
    \caption{Log-likelihood profile for \RpK (left) and \invRpK (right) using ``fake" efficiency to constrain the central value to be equal to unity.}
    \label{fig:simfit_RpK=1_NLL}
\end{figure}

Requirements based on the particle identification probabilities were applied to all the tracks to reduce the backgrounds originating from hadron mis-identification. The remaining components were  then later taken into account in the fit to the invariant mass distributions. 

Besides these sources of background, one has to take into account backgrounds from cascade decays. The branching fraction of \bquark \to \cquark $\ell \nu $  decays is typically three orders of magnitude larger than the \bquark \to \squark one. These types of backgrounds are  not relevant  in the cases where the leptons decay via a resonance like the \jpsi. 

Dedicated vetoes were setup  to suppress some of them, the remaining events are then  modelled in the fit  or taken into account as part of the systematic studies. 

One of the most important aspects of a  LU test is to ensure a good control of the efficiencies; this was achieved as stated earlier thanks to the evaluation of the ratio \invRJPsi computed as: 
\begin{eqnarray}
\label{eq:rjpsi_def_real}
\invRJPsi = \frac{N(\LbTopKJPsiee)}{N(\LbTopKJPsimm)} \times \frac{\epsilon(\LbTopKJPsimm)}{\epsilon(\LbTopKJPsiee)}.
\end{eqnarray}
The aim of this stringent test is to make sure that this ratio is equal to unity and flat across phase-space.  
The simulation is known not to be a perfect description  of the data. A set of ``corrections" derived from data are applied to the simulation to account for these differences.  They are based on the kinematics and decay model of the \Lb particle but also on  the multiplicity of the events. 
The \invRJPsi test was performed separately for each of the trigger categories and data taking  periods.
%For what concerns the muon mode, only one trigger category (\lom) is used. For the electron mode, two default categories are used (\loi and \loeex).
%The notation in this section represents the trigger category of the electron mode, as the muon one is always the same. 

\begin{figure}[!ht]
    \centering
        \includegraphics[height=2.4in]{figs/lu/rjpsi_comparison_nogray_unblind.pdf}
    \caption{Comparison of unblinded \invRJPsi values in different trigger categories and datasets, with total and statistical-only uncertainties displayed.}
    \label{fig:comp_rjpsi_unblind}
\end{figure}
The procedure described below to measure \invRJPsi is identical between the datasets, with the only difference arising from  selection requirements and weights applied to the simulation.
\begin{enumerate}
    \item The \LbTopKJPsimm generator-level simulation sample, with the relevant weights applied, is used to extract the number of simulated events at the generator stage. 
    \item The \LbTopKJPsimm reconstructed-level simulation sample, processed through the complete chain of selection requirements, and having all the relevant weights applied, is used to extract the number of simulated events after the final selection.
    \item The number of reconstructed-level events (step 2) is divided by the number of generated-level events (step 1), and multiplied by the values of generating and filtering efficiencies, to get the total efficiency.
    \item For  Run I, the 2011 and 2012 datasets have to be merged. To do so, their simulation samples are merged, having a dedicated weight applied ensuring the correct ratio of integrated luminosity (1:2) between the two datasets. In addition, the ratio of \Lb production cross-sections at 8 and 7~TeV is taken to be $1.23$, as per the LHCb measurement~\cite{LHCb-PAPER-2015-032}.  
  The   relevant values of generation and filtering efficiencies are passed to each of the two datasets. Steps 1 and 2 are performed with already merged generator-level and reconstruction-level samples.
    \item The simulation samples of the specific backgrounds, with the final selection applied, are used to extract their invariant mass shapes.
    \item The \LbTopKJPsimm simulation sample is used to extract the signal invariant mass shape.
    \item The fit is performed to the  \LbTopKJPsimm data, with the final selection applied. The signal yield and its uncertainty are extracted from the fit.
    \item The signal yield is divided by the total efficiency (step 3) to obtain the efficiency-corrected yield.
    \item All the previous steps are repeated for the \LbTopKJPsiee mode.
    \item Efficiency-corrected yields of the \LbTopKJPsiee are  divided by the efficiency-corrected \LbTopKJPsimm yields to get the value of \invRJPsi.
  \end{enumerate}

Comparisons of \invRJPsi between trigger categories and datasets are shown in Fig.~\ref{fig:comp_rjpsi_unblind}. The uncertainties displayed are statistical uncertainties only.
Getting \invRJPsi ``right" as a function of phase-space, $\invRJPsi = 0.96 \pm 0.05$,  took the best part of a year of Vitalii's PhD.

Finally, \invRpK is measured using a simultaneous fit to both \LbTopKmm and \LbTopKee decay modes, using all available data sets and trigger categories.  The yields of the control modes and the efficiencies are measured beforehand and are plugged as Gaussian constrains in the fit. 
The fit has two observables, \invRpK  and  {$r_{\BR} = \BR(\LbTopKmm)/\BR(\LbTopKJPsimm)$}. The branching fraction of the rare electron mode is later derived as a byproduct of the simultaneous fit. 



\begin{figure}[!ht]
    \centering

        \centering
            \includegraphics[scale=0.6]{figs/lu/Fig5.pdf}
 \caption{Measured value of \invRpK in the range $0.1 < \qsq < 6 \gevgevcccc$ and $\m(\proton\kaon^-)< 2600 \mevcc$ (red point), 
    including statistical and systematic uncertainties, compared to unity (dashed line).}
   
\end{figure}


The result of the test of LU in \LbTopKll decays, \invRpK, in the range \mbox{$0.1 < q^2 < 6 \gevgevcccc$} and \mbox{$m(\proton\kaon^-)< 2600 \mevcc$} is
\begin{equation*}
    \left. \invRpK \right|_{0.1 < q^2 < 6 \gevgevcccc} = 1.17 ^{\,+\,0.18}_{\,-\,0.16} \pm 0.07,
\end{equation*}
where the first uncertainty is statistical and the second systematic.

The first measurement of the branching fraction of the rare muonic decay mode \mbox{\LbTopKmm} is also performed and its value is found to be 
\mbox{$\left. {\BR(\LbTopKmm)}\right|_{0.1 < q^2 < 6 \gevgevcccc} = 
    \left(2.65 \pm 0.14 \pm 0.12 \pm 0.29 ^{\,+\,0.38}_{\,-\,0.23} \right) \times 10^{-7}$}.
    
 The electron mode \LbTopKee is observed for the first time $\left. {\BR(\LbTopKee)}\right|_{0.1 < q^2 < 6 \gevgevcccc} = \left(3.1 \pm0.4 \pm 0.2 \pm 0.3 ^{\,+\,0.4}_{\,-\,0.3} \right) \times 10^{-7}$, 
with a significance larger than $7\sigma$ including systematic uncertainties.

To conclude, more data are needed to confirm or exclude the presence of NP contributions in these decays.
It should be noted that the current analysis is sensitive to   different experimental uncertainties than those of lepton-universality tests performed with \B mesons, such as the backgrounds that affect the extraction of the signal yields from data, or 
the control modes which are used to calibrate the simulation and measure the double ratio. Consequently, it provides an independent test of the SM.

Finally, the prospects for \btosll decays with the LHCb Upgrades are very exciting. 
The statistical uncertainties will be significantly reduced, so that with 23 fb$^{-1}$ we expect to reach about 0.025, 0.031 and 0.076 precision on \RK, \RKst and \RpK respectively~\cite{Aaij:2636441}.  It will also be possible to investigate new \bquark-decay modes, and especially  to explore angular observables, to probe directly the Wilson coefficients and who knows maybe discover New Physics ? 


==> foreword.tex <==

\addcontentsline{toc}{chapter}{Pr\'elude}

%\chapter*{Pr\'elude}
\begin{flushright}
Orsay, August 30$^{th}~2019$
\end{flushright}
I am writing this foreword from an odd place. \invRpK is still blind and hopefully will be unblinded in a few weeks. The expected statistical uncertainty is quite large, about 16\%. However, this measurement will say ``something" about the \bsll anomalies. 
I am lucky to witness a peculiar time, where saying that we might have signs, indications or hints of New Physics in our LHCb data is not a complete fantasy.   
Some of the global flavour fits  to the Wilson coefficients do report up to five standard deviations with respect to the Standard Model predictions. How exciting is that? Can these anomalies be only a misunderstanding of hadronic uncertainties? That would be rubbish. What do we think of the Leptoquarks? What about the somewhat resilient $U_{1}\equiv ({\bf 3}, {\bf 1})_{2/3} $?  \\
It goes without saying that flavour physics analyses are  not just about New Physics searches, far from it, and this humble document aims at demonstrating so. 
Part of me though, always envied my peers who were ``there" when new or unexpected particles were discovered.
Without further ado, let us dive in. \\ 
Trois, quatre...


==> lhcb-symbols-def.tex <==
%%% $Id: lhcb-symbols-def.tex 106630 2017-04-09 10:37:45Z fwilson $
%%% ======================================================================
%%% Purpose: Standard LHCb aliases
%%% Author: Originally Ulrik Egede, adapted by Tomasz Skwarnicki for templates,
%%% rewritten by Chris Parkes
%%% Maintainer : Ulrik Egede (2010 - 2012)
%%% Maintainer : Rolf Oldeman (2012 - 2014)
%%% =======================================================================

%%% To use this file outside the normal LHCb document environment, the
%%% following should be added in a preamble (before \begin{document}
%%%
%%%\usepackage{ifthen} 
%%%\newboolean{uprightparticles}
%%%\setboolean{uprightparticles}{false} %Set true for upright particle symbols
\usepackage{xspace} 
\usepackage{upgreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% The following is to ensure that the template automatically can process
%%% this file.
%%%
%%% Add comments with at least three %%% preceding.
%%% Add new sections with one % preceding
%%% Add new subsections with two %% preceding
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\HybridAlgo{{\tt Hybrid Seeding}\xspace}
%
%Tracks
\def\houghcluster{\texttt{Hough-like Cluster}\xspace}
\def\houghclusters{\texttt{Hough-like Clusters}\xspace}

\def\more{\textgreater\xspace}
\def\less{\textless\xspace}
\def\UpTracks{{\it UpperTrack}\xspace}
\def\DoTracks{{\it DownTrack}\xspace}
\def\betahit{\ensuremath{t_y^{hit}}\xspace}
\def\chidof{\ensuremath{\chi^{2}/ndof}\xspace}

\def\UpModule {{\it UpperModule}\xspace}
\def\DoModule {{\it DownModule}\xspace}
%%%%%%%%%%%%%%
% Algorithm %
%%%%%%%%%%%%%%%%%
\def\Case{{\tt Case}\xspace}
\def\Cases{{\tt Cases}\xspace}
         
\def\forwardtracking {{\it Forward Tracking}\xspace}
\def\seeding {{\it Seeding}\xspace}
\def\mc {{\tt MC}\xspace}
\def\mchit {{\tt MCHit}\xspace}
\def\mchits {{\tt MCHits}\xspace}
\def\cluster {{\tt Cluster}\xspace}
\def\clusters {{\tt Clusters}\xspace}
\def\mcparticle{{\tt MCParticle}\xspace}
\def\lhcbid{{\tt LHCbID}\xspace}
\def\bfield {{B-Field }\xspace}
\def\bsphiphi {{$B_s^0\rightarrow \phi\phi$ }\xspace}
\def\bsphiphikk {{$B_s^0\rightarrow \phi\left(K^{+}K^{-}\right)\phi\left(K^{+}K^{-}\right)$ }\xspace}
\def\yz{{\it y-z}xspace}
\def\xz{{\it x-z}\xspace}
\def\levelT{{\tt lvT}\xspace}
\def\ftchannelID{{\tt FTChannelID}\xspace}
\def\PrHitManager{{\tt PrFTHitManager}\xspace}
%%layers hits
\def\yminHit{{$\mbox{\texttt{Hit}}_{\mbox{\texttt{yMin}}}$}\xspace} 
\def\ymaxHit{{$\mbox{\texttt{Hit}}_{\mbox{\texttt{yMax}}}$}\xspace}
\def\insituysegmentation{{\textit{in-situ y-segmentation}}\xspace}
\def\maxyzero{{\tt maxYatZeroLow}\xspace}
\def\maxyref{{\tt maxYatzRefLow}\xspace}
\def\prhit{{\tt PrHit}\xspace}
\def\prhits{{\tt PrHits}\xspace}
\def\xzplane{{\textit{x-z} plane}\xspace}
\def\yzplane{{\textit{y-z} plane}\xspace}
\def\xzprojections{{\it x-z projections}\xspace}
\def\xzprojection{{\it x-z projection}\xspace}
\def\xzprojectionfit{{\it x-z projection fit}\xspace}
\def\yzprojectionfit{{\it y-z projection fit}\xspace}                      
\def\xhit{{\it x-hit}\xspace}
\def\xhits{{\it x-hits}\xspace}
\def\uhit{{\it u-hit}\xspace}
\def\vhit{{\it v-hit}\xspace}
\def\stereohit{{\it u/v-hit}\xspace}
\def\stereohits{{\it u/v-hits}\xspace}

\def\uvhit{{\it u/v-hit}\xspace}
\def\uvhits{{\it u/v-hits}\xspace}
\def\xlayer{{\it x-layer}\xspace}
\def\xlayers{{\it x-layers}\xspace}
\def\uvlayer{{\it u/v-layer}\xspace}
\def\uvlayers{{\it u/v-layers}\xspace}
\def\stereolayer{{\it u/v-layer}\xspace}
\def\stereolayers{{\it u/v-layers}\xspace}

%\def\twohitcombo {{\it two-hit-combinati}}
 \def\stereoplane{{\it u/v-plane}\xspace}
\def\xfiber{{\it x-fiber}\xspace}
\def\ufiber{{\it u-fiber}\xspace}
\def\vfiber{{\it v-fiber}\xspace}
\def\uvfibers{{\it u/v-fibers}\xspace}
\def\stereoplanes{{\it v planes}\xspace}


\def\twohit {{\it two-hit}\xspace}
\def\threehit{{\it three-hit}\xspace}
\def\threestep{{\it three-step}\xspace}
\def\OldAlgo{{\tt TDR Seeding}\xspace}    
\def\HybridAlgo{{\tt Hybrid Seeding}\xspace}

 
%\def\scifi {{\it Scintillating Fiber}\xspace}
\def\UT{{\it UT}\xspace}
\def\scifitracker{{\it Scintillating Fiber Tracker}\xspace}
\def\scifi{{\it Scintillating Fiber Tracker}\xspace}
\def\ft{{\it FT}\xspace}
\def\velout{{\tt VeloUT}\xspace}
%%%tracking definitions 
\def\reconstructed{{\it reconstructed}\xspace}
\def\reconstructible{{\it reconstructible}\xspace}
\def\ghost{{\it ghost}\xspace}
\def\ghostrate{{\it ghost rate}\xspace} 
                    \def\treff {{\it tracking efficiency}\xspace}
\def\treffs {{\it tracking efficiencies}\xspace}
\def\efficiency{{\it efficiency}\xspace}
\def\purity{{\it purity}\xspace}
\def\hitpurity{{\it hit purity}\xspace}
\def\hitefficiency{{\it hit efficiency}\xspace}
\def\clone {{\it clone}\xspace}
\def\clonerate {{\it clone rate}\xspace}
\def\timing{{\it timing}\xspace}
\def\clones {{\it clones}\xspace}
\def\longtrack {{\tt long track}\xspace}
\def\longtracks {{\tt long tracks}\xspace}
\def\seedtrack {{\tt seed track}\xspace}
\def\hasT {{\tt hasT}\xspace}
\def\hasVelo {{\tt hasVelo}\xspace}
 
%%%default parameters
\def\minpt {{\tt minPT}\xspace}
\def\zmagnetparams {{$z_{Mag,i}$}\xspace}
\def\xparams {{\tt $x_{cor,i}$}\xspace}




\def\sipms{{\it SiPM}\xspace}
\def\sipm{{\it SiPM}\xspace}

\def\maxxwindow {{\tt maxXWindow}\xspace}
\def\maxxwindowslope {{\tt maxXWindowSlope}\xspace}
\def\toly {{\tt tolY}\xspace}
\def\tolyslope {{\tt tolYSlope}\xspace}
\def\mintotalhits {{\tt minTotalHits}\xspace}
\def\byparams {{\tt byParams}\xspace}
\def\cyparams {{\tt cyParams}\xspace}
\def\maxychiatmagnet {{\tt maxYChi2AtMagnet}\xspace}
\def\yqualityweight {{\tt YQualityWeight}\xspace}
\def\deltaquality {{\tt DeltaQuality}\xspace}
\def\maxquality {{\tt MaxQuality}\xspace}
\def\tolymag {{\tt TolYMag}\xspace}
\def\tolymagslope {{\tt TolYMagSlope}\xspace}

\def\maxchilinearfit {{\tt MaxChi2LinearFit}\xspace}
\def\maxchistereo {{\tt MaxChi2Stereo}\xspace}

\def\maxchiperdof {{\tt MaxChi2PerDoF}\xspace} %4
\def\maxchixprojection {{\tt MaxChi2XProjection}\xspace} %9


%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\lhcb {\mbox{LHCb}\xspace}
\def\atlas  {\mbox{ATLAS}\xspace}
\def\cms    {\mbox{CMS}\xspace}
\def\alice  {\mbox{ALICE}\xspace}
\def\babar  {\mbox{BaBar}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\cleo   {\mbox{CLEO}\xspace}
\def\cdf    {\mbox{CDF}\xspace}
\def\dzero  {\mbox{D0}\xspace}
\def\aleph  {\mbox{ALEPH}\xspace}
\def\delphi {\mbox{DELPHI}\xspace}
\def\opal   {\mbox{OPAL}\xspace}
\def\lthree {\mbox{L3}\xspace}
\def\sld    {\mbox{SLD}\xspace}
%%%\def\argus  {\mbox{ARGUS}\xspace}
%%%\def\uaone  {\mbox{UA1}\xspace}
%%%\def\uatwo  {\mbox{UA2}\xspace}
%%%\def\ux85 {\mbox{UX85}\xspace}
\def\cern {\mbox{CERN}\xspace}
\def\lhc    {\mbox{LHC}\xspace}
\def\lep    {\mbox{LEP}\xspace}
\def\tevatron {Tevatron\xspace}

%% LHCb sub-detectors and sub-systems

%%%\def\pu     {PU\xspace}
\def\velo   {VELO\xspace}
\def\rich   {RICH\xspace}
\def\richone {RICH1\xspace}
\def\richtwo {RICH2\xspace}
\def\ttracker {TT\xspace}
\def\intr   {IT\xspace}
\def\st     {ST\xspace}
\def\ot     {OT\xspace}
\def\herschel {\mbox{\textsc{HeRSCheL}}\xspace}
%%%\def\Tone   {T1\xspace}
%%%\def\Ttwo   {T2\xspace}
%%%\def\Tthree {T3\xspace}
%%%\def\Mone   {M1\xspace}
%%%\def\Mtwo   {M2\xspace}
%%%\def\Mthree {M3\xspace}
%%%\def\Mfour  {M4\xspace}
%%%\def\Mfive  {M5\xspace}
\def\spd    {SPD\xspace}
\def\presh  {PS\xspace}
\def\ecal   {ECAL\xspace}
\def\hcal   {HCAL\xspace}
%%%\def\bcm    {BCM\xspace}
\def\MagUp {\mbox{\em Mag\kern -0.05em Up}\xspace}
\def\MagDown {\mbox{\em MagDown}\xspace}

\def\ode    {ODE\xspace}
\def\daq    {DAQ\xspace}
\def\tfc    {TFC\xspace}
\def\ecs    {ECS\xspace}
\def\lone   {L0\xspace}
\def\hlt    {HLT\xspace}
\def\hltone {HLT1\xspace}
\def\hlttwo {HLT2\xspace}

%%% Upright (not slanted) Particles

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 
 
 %\mathchardef\Deltares="7101
 %\mathchardef\Xi="7104
 %\mathchardef\Lambda="7103
 %\mathchardef\Sigma="7106
 %\mathchardef\Omega="710A


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Particles
\makeatletter
\ifcase \@ptsize \relax% 10pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{4}{5}}% \tiny: 5/6
\or% 11pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\or% 12pt
  \newcommand{\miniscule}{\@setfontsize\miniscule{5}{6}}% \tiny: 6/7
\fi
\makeatother


\DeclareRobustCommand{\optbar}[1]{\shortstack{{\miniscule (\rule[.5ex]{1.25em}{.18mm})}
  \\ [-.7ex] $#1$}}


%% Leptons

\let\emi\en
\def\electron   {{\ensuremath{\Pe}}\xspace}
\def\en         {{\ensuremath{\Pe^-}}\xspace}   % electron negative (\em is taken)
\def\ep         {{\ensuremath{\Pe^+}}\xspace}
\def\epm        {{\ensuremath{\Pe^\pm}}\xspace} 
\def\epem       {{\ensuremath{\Pe^+\Pe^-}}\xspace}
%%%\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\muon       {{\ensuremath{\Pmu}}\xspace}
\def\mup        {{\ensuremath{\Pmu^+}}\xspace}
\def\mun        {{\ensuremath{\Pmu^-}}\xspace} % muon negative (\mum is taken)
\def\mumu       {{\ensuremath{\Pmu^+\Pmu^-}}\xspace}

\def\tauon      {{\ensuremath{\Ptau}}\xspace}
\def\taup       {{\ensuremath{\Ptau^+}}\xspace}
\def\taum       {{\ensuremath{\Ptau^-}}\xspace}
\def\tautau     {{\ensuremath{\Ptau^+\Ptau^-}}\xspace}

\def\lepton     {{\ensuremath{\ell}}\xspace}
\def\ellm       {{\ensuremath{\ell^-}}\xspace}
\def\ellp       {{\ensuremath{\ell^+}}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {{\ensuremath{\Pnu}}\xspace}
\def\neub       {{\ensuremath{\overline{\Pnu}}}\xspace}
%%%\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {{\ensuremath{\neu_e}}\xspace}
\def\neueb      {{\ensuremath{\neub_e}}\xspace}
%%%\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {{\ensuremath{\neu_\mu}}\xspace}
\def\neumb      {{\ensuremath{\neub_\mu}}\xspace}
%%%\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {{\ensuremath{\neu_\tau}}\xspace}
\def\neutb      {{\ensuremath{\neub_\tau}}\xspace}
%%%\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {{\ensuremath{\neu_\ell}}\xspace}
\def\neulb      {{\ensuremath{\neub_\ell}}\xspace}
%%%\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {{\ensuremath{\Pgamma}}\xspace}
\def\H      {{\ensuremath{\PH^0}}\xspace}
\def\Hp     {{\ensuremath{\PH^+}}\xspace}
\def\Hm     {{\ensuremath{\PH^-}}\xspace}
\def\Hpm    {{\ensuremath{\PH^\pm}}\xspace}
\def\W      {{\ensuremath{\PW}}\xspace}
\def\Wp     {{\ensuremath{\PW^+}}\xspace}
\def\Wm     {{\ensuremath{\PW^-}}\xspace}
\def\Wpm    {{\ensuremath{\PW^\pm}}\xspace}
\def\Z      {{\ensuremath{\PZ}}\xspace}

%% Quarks

\def\quark     {{\ensuremath{\Pq}}\xspace}
\def\quarkbar  {{\ensuremath{\overline \quark}}\xspace}
\def\qqbar     {{\ensuremath{\quark\quarkbar}}\xspace}
\def\uquark    {{\ensuremath{\Pu}}\xspace}
\def\uquarkbar {{\ensuremath{\overline \uquark}}\xspace}
\def\uubar     {{\ensuremath{\uquark\uquarkbar}}\xspace}
\def\dquark    {{\ensuremath{\Pd}}\xspace}
\def\dquarkbar {{\ensuremath{\overline \dquark}}\xspace}
\def\ddbar     {{\ensuremath{\dquark\dquarkbar}}\xspace}
\def\squark    {{\ensuremath{\Ps}}\xspace}
\def\squarkbar {{\ensuremath{\overline \squark}}\xspace}
\def\ssbar     {{\ensuremath{\squark\squarkbar}}\xspace}
\def\cquark    {{\ensuremath{\Pc}}\xspace}
\def\cquarkbar {{\ensuremath{\overline \cquark}}\xspace}
\def\ccbar     {{\ensuremath{\cquark\cquarkbar}}\xspace}
\def\bquark    {{\ensuremath{\Pb}}\xspace}
\def\bquarkbar {{\ensuremath{\overline \bquark}}\xspace}
\def\bbbar     {{\ensuremath{\bquark\bquarkbar}}\xspace}
\def\tquark    {{\ensuremath{\Pt}}\xspace}
\def\tquarkbar {{\ensuremath{\overline \tquark}}\xspace}
\def\ttbar     {{\ensuremath{\tquark\tquarkbar}}\xspace}

%% Light mesons

\def\hadron {{\ensuremath{\Ph}}\xspace}
\def\pion   {{\ensuremath{\Ppi}}\xspace}
\def\piz    {{\ensuremath{\pion^0}}\xspace}
\def\pizs   {{\ensuremath{\pion^0\mbox\,\mathrm{s}}}\xspace}
\def\pip    {{\ensuremath{\pion^+}}\xspace}
\def\pim    {{\ensuremath{\pion^-}}\xspace}
\def\pipm   {{\ensuremath{\pion^\pm}}\xspace}
\def\pimp   {{\ensuremath{\pion^\mp}}\xspace}

\def\rhomeson {{\ensuremath{\Prho}}\xspace}
\def\rhoz     {{\ensuremath{\rhomeson^0}}\xspace}
\def\rhop     {{\ensuremath{\rhomeson^+}}\xspace}
\def\rhom     {{\ensuremath{\rhomeson^-}}\xspace}
\def\rhopm    {{\ensuremath{\rhomeson^\pm}}\xspace}
\def\rhomp    {{\ensuremath{\rhomeson^\mp}}\xspace}

\def\kaon    {{\ensuremath{\PK}}\xspace}
%%% do NOT use ensuremath here
  \def\Kbar    {{\kern 0.2em\overline{\kern -0.2em \PK}{}}\xspace}
\def\Kb      {{\ensuremath{\Kbar}}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}
\def\Kz      {{\ensuremath{\kaon^0}}\xspace}
\def\Kzb     {{\ensuremath{\Kbar{}^0}}\xspace}
\def\Kp      {{\ensuremath{\kaon^+}}\xspace}
\def\Km      {{\ensuremath{\kaon^-}}\xspace}
\def\Kpm     {{\ensuremath{\kaon^\pm}}\xspace}
\def\Kmp     {{\ensuremath{\kaon^\mp}}\xspace}
\def\KS      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle S}}}}\xspace}
\def\KL      {{\ensuremath{\kaon^0_{\mathrm{ \scriptscriptstyle L}}}}\xspace}
\def\Kstarz  {{\ensuremath{\kaon^{*0}}}\xspace}
\def\Kstarzb {{\ensuremath{\Kbar{}^{*0}}}\xspace}
\def\Kstar   {{\ensuremath{\kaon^*}}\xspace}
\def\Kstarb  {{\ensuremath{\Kbar{}^*}}\xspace}
\def\Kstarp  {{\ensuremath{\kaon^{*+}}}\xspace}
\def\Kstarm  {{\ensuremath{\kaon^{*-}}}\xspace}
\def\Kstarpm {{\ensuremath{\kaon^{*\pm}}}\xspace}
\def\Kstarmp {{\ensuremath{\kaon^{*\mp}}}\xspace}

\newcommand{\etaz}{\ensuremath{\Peta}\xspace}
\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}
\newcommand{\phiz}{\ensuremath{\Pphi}\xspace}
\newcommand{\omegaz}{\ensuremath{\Pomega}\xspace}

%% Heavy mesons

%%% do NOT use ensuremath here
  \def\Dbar    {{\kern 0.2em\overline{\kern -0.2em \PD}{}}\xspace}
\def\D       {{\ensuremath{\PD}}\xspace}
\def\Db      {{\ensuremath{\Dbar}}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\Dz      {{\ensuremath{\D^0}}\xspace}
\def\Dzb     {{\ensuremath{\Dbar{}^0}}\xspace}
\def\Dp      {{\ensuremath{\D^+}}\xspace}
\def\Dm      {{\ensuremath{\D^-}}\xspace}
\def\Dpm     {{\ensuremath{\D^\pm}}\xspace}
\def\Dmp     {{\ensuremath{\D^\mp}}\xspace}
\def\Dstar   {{\ensuremath{\D^*}}\xspace}
\def\Dstarb  {{\ensuremath{\Dbar{}^*}}\xspace}
\def\Dstarz  {{\ensuremath{\D^{*0}}}\xspace}
\def\Dstarzb {{\ensuremath{\Dbar{}^{*0}}}\xspace}
\def\Dstarp  {{\ensuremath{\D^{*+}}}\xspace}
\def\Dstarm  {{\ensuremath{\D^{*-}}}\xspace}
\def\Dstarpm {{\ensuremath{\D^{*\pm}}}\xspace}
\def\Dstarmp {{\ensuremath{\D^{*\mp}}}\xspace}
\def\Ds      {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsp     {{\ensuremath{\D^+_\squark}}\xspace}
\def\Dsm     {{\ensuremath{\D^-_\squark}}\xspace}
\def\Dspm    {{\ensuremath{\D^{\pm}_\squark}}\xspace}
\def\Dsmp    {{\ensuremath{\D^{\mp}_\squark}}\xspace}
\def\Dss     {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssp    {{\ensuremath{\D^{*+}_\squark}}\xspace}
\def\Dssm    {{\ensuremath{\D^{*-}_\squark}}\xspace}
\def\Dsspm   {{\ensuremath{\D^{*\pm}_\squark}}\xspace}
\def\Dssmp   {{\ensuremath{\D^{*\mp}_\squark}}\xspace}

\def\B       {{\ensuremath{\PB}}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {{\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}}\xspace}
\def\Bb      {{\ensuremath{\Bbar}}\xspace}
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\Bz      {{\ensuremath{\B^0}}\xspace}
\def\Bzb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bu      {{\ensuremath{\B^+}}\xspace}
\def\Bub     {{\ensuremath{\B^-}}\xspace}
\def\Bp      {{\ensuremath{\Bu}}\xspace}
\def\Bm      {{\ensuremath{\Bub}}\xspace}
\def\Bpm     {{\ensuremath{\B^\pm}}\xspace}
\def\Bmp     {{\ensuremath{\B^\mp}}\xspace}
\def\Bd      {{\ensuremath{\B^0}}\xspace}
\def\Bs      {{\ensuremath{\B^0_\squark}}\xspace}
\def\Bsb     {{\ensuremath{\Bbar{}^0_\squark}}\xspace}
\def\Bdb     {{\ensuremath{\Bbar{}^0}}\xspace}
\def\Bc      {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcp     {{\ensuremath{\B_\cquark^+}}\xspace}
\def\Bcm     {{\ensuremath{\B_\cquark^-}}\xspace}
\def\Bcpm    {{\ensuremath{\B_\cquark^\pm}}\xspace}

%% Onia

\def\jpsi     {{\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}}\xspace}
\def\psitwos  {{\ensuremath{\Ppsi{(2S)}}}\xspace}
\def\psiprpr  {{\ensuremath{\Ppsi(3770)}}\xspace}
\def\etac     {{\ensuremath{\Peta_\cquark}}\xspace}
\def\chiczero {{\ensuremath{\Pchi_{\cquark 0}}}\xspace}
\def\chicone  {{\ensuremath{\Pchi_{\cquark 1}}}\xspace}
\def\chictwo  {{\ensuremath{\Pchi_{\cquark 2}}}\xspace}
  %\mathchardef\Upsilon="7107
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {{\Y1S}}
\def\TwoS  {{\Y2S}}
\def\ThreeS{{\Y3S}}
\def\FourS {{\Y4S}}
\def\FiveS {{\Y5S}}

\def\chic  {{\ensuremath{\Pchi_{c}}}\xspace}

%% Baryons

\def\proton      {{\ensuremath{\Pp}}\xspace}
\def\antiproton  {{\ensuremath{\overline \proton}}\xspace}
\def\neutron     {{\ensuremath{\Pn}}\xspace}
\def\antineutron {{\ensuremath{\overline \neutron}}\xspace}
\def\Deltares    {{\ensuremath{\PDelta}}\xspace}
\def\Deltaresbar {{\ensuremath{\overline \Deltares}}\xspace}
\def\Xires       {{\ensuremath{\PXi}}\xspace}
\def\Xiresbar    {{\ensuremath{\overline \Xires}}\xspace}
\def\Lz          {{\ensuremath{\PLambda}}\xspace}
\def\Lbar        {{\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}}\xspace}
\def\LorLbar    {\kern 0.18em\optbar{\kern -0.18em \PLambda}{}\xspace}
\def\Lambdares   {{\ensuremath{\PLambda}}\xspace}
\def\Lambdaresbar{{\ensuremath{\Lbar}}\xspace}
\def\Sigmares    {{\ensuremath{\PSigma}}\xspace}
\def\Sigmaresbar {{\ensuremath{\overline \Sigmares}}\xspace}
\def\Sigmaresbarz {{\ensuremath{\Sigmaresbar{}^0}}\xspace}
\def\Omegares    {{\ensuremath{\POmega}}\xspace}
\def\Omegaresbar {{\ensuremath{\overline \POmega}}\xspace}

%%% do NOT use ensuremath here
 % \def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
 % \def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
 % \def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
 % \def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
 % \def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
 % \def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\Lb      {{\ensuremath{\Lz^0_\bquark}}\xspace}
\def\Lbbar   {{\ensuremath{\Lbar{}^0_\bquark}}\xspace}
\def\Lc      {{\ensuremath{\Lz^+_\cquark}}\xspace}
\def\Lcbar   {{\ensuremath{\Lbar{}^-_\cquark}}\xspace}
\def\Xib     {{\ensuremath{\Xires_\bquark}}\xspace}
\def\Xibz    {{\ensuremath{\Xires^0_\bquark}}\xspace}
\def\Xibm    {{\ensuremath{\Xires^-_\bquark}}\xspace}
\def\Xibbar  {{\ensuremath{\Xiresbar{}_\bquark}}\xspace}
\def\Xibbarz {{\ensuremath{\Xiresbar{}_\bquark^0}}\xspace}
\def\Xibbarp {{\ensuremath{\Xiresbar{}_\bquark^+}}\xspace}
\def\Xic     {{\ensuremath{\Xires_\cquark}}\xspace}
\def\Xicz    {{\ensuremath{\Xires^0_\cquark}}\xspace}
\def\Xicp    {{\ensuremath{\Xires^+_\cquark}}\xspace}
\def\Xicbar  {{\ensuremath{\Xiresbar{}_\cquark}}\xspace}
\def\Xicbarz {{\ensuremath{\Xiresbar{}_\cquark^0}}\xspace}
\def\Xicbarm {{\ensuremath{\Xiresbar{}_\cquark^-}}\xspace}
\def\Omegac    {{\ensuremath{\Omegares^0_\cquark}}\xspace}
\def\Omegacbar {{\ensuremath{\Omegaresbar{}_\cquark^0}}\xspace}
\def\Omegab    {{\ensuremath{\Omegares^-_\bquark}}\xspace}
\def\Omegabbar {{\ensuremath{\Omegaresbar{}_\bquark^+}}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\mathcal{B}}}\xspace}
\def\BRvis      {{\ensuremath{\BR_{\mathrm{{vis}}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% Lifetimes
\newcommand{\tauBs}{{\ensuremath{\tau_{\Bs}}}\xspace}
\newcommand{\tauBd}{{\ensuremath{\tau_{\Bd}}}\xspace}
\newcommand{\tauBz}{{\ensuremath{\tau_{\Bz}}}\xspace}
\newcommand{\tauBu}{{\ensuremath{\tau_{\Bp}}}\xspace}
\newcommand{\tauDp}{{\ensuremath{\tau_{\Dp}}}\xspace}
\newcommand{\tauDz}{{\ensuremath{\tau_{\Dz}}}\xspace}
\newcommand{\tauL}{{\ensuremath{\tau_{\mathrm{ L}}}}\xspace}
\newcommand{\tauH}{{\ensuremath{\tau_{\mathrm{ H}}}}\xspace}

%% Masses
\newcommand{\mBd}{{\ensuremath{m_{\Bd}}}\xspace}
\newcommand{\mBp}{{\ensuremath{m_{\Bp}}}\xspace}
\newcommand{\mBs}{{\ensuremath{m_{\Bs}}}\xspace}
\newcommand{\mBc}{{\ensuremath{m_{\Bc}}}\xspace}
\newcommand{\mLb}{{\ensuremath{m_{\Lb}}}\xspace}

%% EW theory, groups
\def\grpsuthree {{\ensuremath{\mathrm{SU}(3)}}\xspace}
\def\grpsutw    {{\ensuremath{\mathrm{SU}(2)}}\xspace}
\def\grpuone    {{\ensuremath{\mathrm{U}(1)}}\xspace}

\def\ssqtw   {{\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\csqtw   {{\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}}\xspace}
\def\stw     {{\ensuremath{\sin\theta_{\mathrm{W}}}}\xspace}
\def\ctw     {{\ensuremath{\cos\theta_{\mathrm{W}}}}\xspace}
\def\ssqtwef {{\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\csqtwef {{\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\stwef   {{\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\ctwef   {{\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}}\xspace}
\def\gv      {{\ensuremath{g_{\mbox{\tiny V}}}}\xspace}
\def\ga      {{\ensuremath{g_{\mbox{\tiny A}}}}\xspace}

\def\order   {{\ensuremath{\mathcal{O}}}\xspace}
\def\ordalph {{\ensuremath{\mathcal{O}(\alpha)}}\xspace}
\def\ordalsq {{\ensuremath{\mathcal{O}(\alpha^{2})}}\xspace}
\def\ordalcb {{\ensuremath{\mathcal{O}(\alpha^{3})}}\xspace}

%% QCD parameters
\newcommand{\as}{{\ensuremath{\alpha_s}}\xspace}
\newcommand{\MSb}{{\ensuremath{\overline{\mathrm{MS}}}}\xspace}
\newcommand{\lqcd}{{\ensuremath{\Lambda_{\mathrm{QCD}}}}\xspace}
\def\qsq       {{\ensuremath{q^2}}\xspace}

%% CKM, CP violation

\def\eps   {{\ensuremath{\varepsilon}}\xspace}
\def\epsK  {{\ensuremath{\varepsilon_K}}\xspace}
\def\epsB  {{\ensuremath{\varepsilon_B}}\xspace}
\def\epsp  {{\ensuremath{\varepsilon^\prime_K}}\xspace}

\def\CP                {{\ensuremath{C\!P}}\xspace}
\def\CPT               {{\ensuremath{C\!PT}}\xspace}

\def\rhobar {{\ensuremath{\overline \rho}}\xspace}
\def\etabar {{\ensuremath{\overline \eta}}\xspace}

\def\Vud  {{\ensuremath{V_{\uquark\dquark}}}\xspace}
\def\Vcd  {{\ensuremath{V_{\cquark\dquark}}}\xspace}
\def\Vtd  {{\ensuremath{V_{\tquark\dquark}}}\xspace}
\def\Vus  {{\ensuremath{V_{\uquark\squark}}}\xspace}
\def\Vcs  {{\ensuremath{V_{\cquark\squark}}}\xspace}
\def\Vts  {{\ensuremath{V_{\tquark\squark}}}\xspace}
\def\Vub  {{\ensuremath{V_{\uquark\bquark}}}\xspace}
\def\Vcb  {{\ensuremath{V_{\cquark\bquark}}}\xspace}
\def\Vtb  {{\ensuremath{V_{\tquark\bquark}}}\xspace}
\def\Vuds  {{\ensuremath{V_{\uquark\dquark}^\ast}}\xspace}
\def\Vcds  {{\ensuremath{V_{\cquark\dquark}^\ast}}\xspace}
\def\Vtds  {{\ensuremath{V_{\tquark\dquark}^\ast}}\xspace}
\def\Vuss  {{\ensuremath{V_{\uquark\squark}^\ast}}\xspace}
\def\Vcss  {{\ensuremath{V_{\cquark\squark}^\ast}}\xspace}
\def\Vtss  {{\ensuremath{V_{\tquark\squark}^\ast}}\xspace}
\def\Vubs  {{\ensuremath{V_{\uquark\bquark}^\ast}}\xspace}
\def\Vcbs  {{\ensuremath{V_{\cquark\bquark}^\ast}}\xspace}
\def\Vtbs  {{\ensuremath{V_{\tquark\bquark}^\ast}}\xspace}

%% Oscillations

\newcommand{\dm}{{\ensuremath{\Delta m}}\xspace}
\newcommand{\dms}{{\ensuremath{\Delta m_{\squark}}}\xspace}
\newcommand{\dmd}{{\ensuremath{\Delta m_{\dquark}}}\xspace}
\newcommand{\DG}{{\ensuremath{\Delta\Gamma}}\xspace}
\newcommand{\DGs}{{\ensuremath{\Delta\Gamma_{\squark}}}\xspace}
\newcommand{\DGd}{{\ensuremath{\Delta\Gamma_{\dquark}}}\xspace}
\newcommand{\Gs}{{\ensuremath{\Gamma_{\squark}}}\xspace}
\newcommand{\Gd}{{\ensuremath{\Gamma_{\dquark}}}\xspace}
\newcommand{\MBq}{{\ensuremath{M_{\B_\quark}}}\xspace}
\newcommand{\DGq}{{\ensuremath{\Delta\Gamma_{\quark}}}\xspace}
\newcommand{\Gq}{{\ensuremath{\Gamma_{\quark}}}\xspace}
\newcommand{\dmq}{{\ensuremath{\Delta m_{\quark}}}\xspace}
\newcommand{\GL}{{\ensuremath{\Gamma_{\mathrm{ L}}}}\xspace}
\newcommand{\GH}{{\ensuremath{\Gamma_{\mathrm{ H}}}}\xspace}
\newcommand{\DGsGs}{{\ensuremath{\Delta\Gamma_{\squark}/\Gamma_{\squark}}}\xspace}
\newcommand{\Delm}{{\mbox{$\Delta m $}}\xspace}
\newcommand{\ACP}{{\ensuremath{{\mathcal{A}}^{\CP}}}\xspace}
\newcommand{\Adir}{{\ensuremath{{\mathcal{A}}^{\mathrm{ dir}}}}\xspace}
\newcommand{\Amix}{{\ensuremath{{\mathcal{A}}^{\mathrm{ mix}}}}\xspace}
\newcommand{\ADelta}{{\ensuremath{{\mathcal{A}}^\Delta}}\xspace}
\newcommand{\phid}{{\ensuremath{\phi_{\dquark}}}\xspace}
\newcommand{\sinphid}{{\ensuremath{\sin\!\phid}}\xspace}
\newcommand{\phis}{{\ensuremath{\phi_{\squark}}}\xspace}
\newcommand{\betas}{{\ensuremath{\beta_{\squark}}}\xspace}
\newcommand{\sbetas}{{\ensuremath{\sigma(\beta_{\squark})}}\xspace}
\newcommand{\stbetas}{{\ensuremath{\sigma(2\beta_{\squark})}}\xspace}
\newcommand{\stphis}{{\ensuremath{\sigma(\phi_{\squark})}}\xspace}
\newcommand{\sinphis}{{\ensuremath{\sin\!\phis}}\xspace}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\mathrm{ det}}}}\xspace}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\mathrm{ rec/det}}}}\xspace}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\mathrm{ sel/rec}}}}\xspace}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\mathrm{ trg/sel}}}}\xspace}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\mathrm{ tot}}}}\xspace}

\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\wcomb}{\ensuremath{\omega^{\mathrm{comb}}}\xspace}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\mathrm{tag}}}}\xspace}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\mathrm{tag}}^{\mathrm{comb}}}}\xspace}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\mathrm{eff}}}\xspace}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\mathrm{eff}}^{\mathrm{comb}}}\xspace}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}\xspace}
\newcommand{\effD}{{\ensuremath{\etag D^2}}\xspace}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{Pr}}}}\xspace}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\mathrm{ tag}}^{\mathrm{LL}}}}\xspace}

%% Key decay channels

\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}}

\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}

\def\BsPhiGam     {\decay{\Bs}{\phi \g}}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph'^-}}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}}

%% Rare decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}}
\def\bsll     {\decay{\bquark}{\squark \ell^+ \ell^-}}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\FL       {\ensuremath{F_{\mathrm{L}}}\xspace}
\def\AT#1     {\ensuremath{A_{\mathrm{T}}^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\bquark}{\squark \g}}
\def\btodgam  {\decay{\bquark}{\dquark \g}}
\def\Bsmm     {\decay{\Bs}{\mup\mun}}
\def\Bdmm     {\decay{\Bd}{\mup\mun}}
\def\ctl       {\ensuremath{\cos{\theta_\ell}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}\xspace}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}\xspace}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}\xspace}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}\xspace}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}\xspace}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}\xspace}                    % 7

%% Charm

\def\xprime     {\ensuremath{x^{\prime}}\xspace}
\def\yprime     {\ensuremath{y^{\prime}}\xspace}
\def\ycp        {\ensuremath{y_{\CP}}\xspace}
\def\agamma     {\ensuremath{A_{\Gamma}}\xspace}
%%%\def\kpi        {\ensuremath{\PK\Ppi}\xspace}
%%%\def\kk         {\ensuremath{\PK\PK}\xspace}
%%%\def\dkpi       {\decay{\PD}{\PK\Ppi}}
%%%\def\dkk        {\decay{\PD}{\PK\PK}}
\def\dkpicf     {\decay{\Dz}{\Km\pip}}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\mathrm{ \,#1}}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ifthenelse{\boolean{inbibliography}}{\ensuremath{~T\kern -0.05em eV}}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\mathrm{ \,km}}\xspace}
\def\m    {\ensuremath{\mathrm{ \,m}}\xspace}
\def\ma   {\ensuremath{{\mathrm{ \,m}}^2}\xspace}
\def\cm   {\ensuremath{\mathrm{ \,cm}}\xspace}
\def\cma  {\ensuremath{{\mathrm{ \,cm}}^2}\xspace}
\def\mm   {\ensuremath{\mathrm{ \,mm}}\xspace}
\def\mma  {\ensuremath{{\mathrm{ \,mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\upmu\mathrm{m}}}\xspace}
\def\muma {\ensuremath{{\,\upmu\mathrm{m}^2}}\xspace}
\def\nm   {\ensuremath{\mathrm{ \,nm}}\xspace}
\def\fm   {\ensuremath{\mathrm{ \,fm}}\xspace}
\def\barn{\ensuremath{\mathrm{ \,b}}\xspace}
%%%\def\barnhyph{\ensuremath{\mathrm{ -b}}\xspace}
\def\mbarn{\ensuremath{\mathrm{ \,mb}}\xspace}
\def\mub{\ensuremath{{\mathrm{ \,\upmu b}}}\xspace}
%%%\def\mbarnhyph{\ensuremath{\mathrm{ -mb}}\xspace}
\def\nb {\ensuremath{\mathrm{ \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\mathrm{ \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\mathrm{{\,s}}}\xspace}
\def\ms   {\ensuremath{{\mathrm{ \,ms}}}\xspace}
\def\mus  {\ensuremath{{\,\upmu{\mathrm{ s}}}}\xspace}
\def\ns   {\ensuremath{{\mathrm{ \,ns}}}\xspace}
\def\ps   {\ensuremath{{\mathrm{ \,ps}}}\xspace}
\def\fs   {\ensuremath{\mathrm{ \,fs}}\xspace}

\def\mhz  {\ensuremath{{\mathrm{ \,MHz}}}\xspace}
\def\khz  {\ensuremath{{\mathrm{ \,kHz}}}\xspace}
\def\hz   {\ensuremath{{\mathrm{ \,Hz}}}\xspace}

\def\invps{\ensuremath{{\mathrm{ \,ps^{-1}}}}\xspace}
\def\invns{\ensuremath{{\mathrm{ \,ns^{-1}}}}\xspace}

\def\yr   {\ensuremath{\mathrm{ \,yr}}\xspace}
\def\hr   {\ensuremath{\mathrm{ \,hr}}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\mathrm{ K}}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\mathrm{ \,n_{eq}}}\xspace}
\def\neqcmcm {\ensuremath{\mathrm{ \,n_{eq} / cm^2}}\xspace}
\def\kRad {\ensuremath{\mathrm{ \,kRad}}\xspace}
\def\MRad {\ensuremath{\mathrm{ \,MRad}}\xspace}
\def\ci {\ensuremath{\mathrm{ \,Ci}}\xspace}
\def\mci {\ensuremath{\mathrm{ \,mCi}}\xspace}

%% Uncertainties
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\newcommand{\stat}{\ensuremath{\mathrm{\,(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{\,(syst)}}\xspace}

%% Maths

\def\order{{\ensuremath{\mathcal{O}}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chi^2/\mathrm{ndf}}\xspace}
\newcommand{\chisqip}{\ensuremath{\chi^2_{\text{IP}}}\xspace}
\newcommand{\chisqvs}{\ensuremath{\chi^2_{\text{VS}}}\xspace}
\newcommand{\chisqvtx}{\ensuremath{\chi^2_{\text{vtx}}}\xspace}
\newcommand{\chisqvtxndf}{\ensuremath{\chi^2_{\text{vtx}}/\mathrm{ndf}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\PDF {PDF\xspace}

\def\sPlot{\mbox{\em sPlot}\xspace}
%%%\def\sWeight{\mbox{\em sWeight}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_{\mathrm{ T}}$}\xspace}
\def\et         {\mbox{$E_{\mathrm{ T}}$}\xspace}
\def\mt         {\mbox{$M_{\mathrm{ T}}$}\xspace}
\def\dpp        {\ensuremath{\Delta p/p}\xspace}
\def\msq        {\ensuremath{m^2}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%% PID

\def\dllkpi     {\ensuremath{\mathrm{DLL}_{\kaon\pion}}\xspace}
\def\dllppi     {\ensuremath{\mathrm{DLL}_{\proton\pion}}\xspace}
\def\dllepi     {\ensuremath{\mathrm{DLL}_{\electron\pion}}\xspace}
\def\dllmupi    {\ensuremath{\mathrm{DLL}_{\muon\pi}}\xspace}

%% Geometry
%%%\def\mphi       {\mbox{$\phi$}\xspace}
%%%\def\mtheta     {\mbox{$\theta$}\xspace}
%%%\def\ctheta     {\mbox{$\cos\theta$}\xspace}
%%%\def\stheta     {\mbox{$\sin\theta$}\xspace}
%%%\def\ttheta     {\mbox{$\tan\theta$}\xspace}

\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\mathrm{ \,krad}}\xspace}
\def\mrad{\ensuremath{\mathrm{ \,mrad}}\xspace}
\def\rad{\ensuremath{\mathrm{ \,rad}}\xspace}

%% Accelerator
\def\betastar {\ensuremath{\beta^*}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\intlum}[1]{\ensuremath{\int\lum=#1}\xspace}  % {2 \,\invfb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
%%%\def\ansys      {\mbox{\textsc{Ansys}}\xspace}
\def\bcvegpy    {\mbox{\textsc{Bcvegpy}}\xspace}
\def\boole      {\mbox{\textsc{Boole}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\dirac      {\mbox{\textsc{Dirac}}\xspace}
%%%\def\erasmus    {\mbox{\textsc{Erasmus}}\xspace}
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\fewz       {\mbox{\textsc{Fewz}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
%%%\def\garfield   {\mbox{\textsc{Garfield}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\geant      {\mbox{\textsc{Geant4}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\herwig     {\mbox{\textsc{Herwig}}\xspace}
\def\moore      {\mbox{\textsc{Moore}}\xspace}
\def\neurobayes {\mbox{\textsc{NeuroBayes}}\xspace}
\def\photos     {\mbox{\textsc{Photos}}\xspace}
\def\powheg     {\mbox{\textsc{Powheg}}\xspace}
%%%\def\pyroot     {\mbox{\textsc{PyRoot}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\resbos     {\mbox{\textsc{ResBos}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\spice      {\mbox{\textsc{Spice}}\xspace}
%%%\def\tosca      {\mbox{\textsc{Tosca}}\xspace}
\def\urania     {\mbox{\textsc{Urania}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
%%%\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}
\def\svn        {\mbox{\textsc{SVN}}\xspace}

%% Data processing
\def\kbytes     {\ensuremath{{\mathrm{ \,kbytes}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbytes/s}}}\xspace}
\def\kbits      {\ensuremath{{\mathrm{ \,kbits}}}\xspace}
\def\kbsps      {\ensuremath{{\mathrm{ \,kbits/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbits/s}}}\xspace}
\def\mbytes     {\ensuremath{{\mathrm{ \,Mbytes}}}\xspace}
\def\mbps       {\ensuremath{{\mathrm{ \,Mbyte/s}}}\xspace}
\def\mbsps      {\ensuremath{{\mathrm{ \,Mbytes/s}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbits/s}}}\xspace}
\def\gbytes     {\ensuremath{{\mathrm{ \,Gbytes}}}\xspace}
\def\gbsps      {\ensuremath{{\mathrm{ \,Gbytes/s}}}\xspace}
\def\tbytes     {\ensuremath{{\mathrm{ \,Tbytes}}}\xspace}
\def\tbpy       {\ensuremath{{\mathrm{ \,Tbytes/yr}}}\xspace}

\def\dst        {DST\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Detector related
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Detector technologies
\def\nonn {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\ponn {\ensuremath{\mathrm{{ \mathit{p^+}} \mbox{-} on\mbox{-}{ \mathit{n}}}}\xspace}
\def\nonp {\ensuremath{\mathrm{{ \mathit{n^+}} \mbox{-} on\mbox{-}{ \mathit{p}}}}\xspace}
\def\cvd  {CVD\xspace}
\def\mwpc {MWPC\xspace}
\def\gem  {GEM\xspace}

%% Detector components, electronics
\def\tell1  {TELL1\xspace}
\def\ukl1   {UKL1\xspace}
\def\beetle {Beetle\xspace}
\def\otis   {OTIS\xspace}
\def\croc   {CROC\xspace}
\def\carioca {CARIOCA\xspace}
\def\dialog {DIALOG\xspace}
\def\sync   {SYNC\xspace}
\def\cardiac {CARDIAC\xspace}
\def\gol    {GOL\xspace}
\def\vcsel  {VCSEL\xspace}
\def\ttc    {TTC\xspace}
\def\ttcrx  {TTCrx\xspace}
\def\hpd    {HPD\xspace}
\def\pmt    {PMT\xspace}
\def\specs  {SPECS\xspace}
\def\elmb   {ELMB\xspace}
\def\fpga   {FPGA\xspace}
\def\plc    {PLC\xspace}
\def\rasnik {RASNIK\xspace}
\def\elmb   {ELMB\xspace}
\def\can    {CAN\xspace}
\def\lvds   {LVDS\xspace}
\def\ntc    {NTC\xspace}
\def\adc    {ADC\xspace}
\def\led    {LED\xspace}
\def\ccd    {CCD\xspace}
\def\hv     {HV\xspace}
\def\lv     {LV\xspace}
\def\pvss   {PVSS\xspace}
\def\cmos   {CMOS\xspace}
\def\fifo   {FIFO\xspace}
\def\ccpc   {CCPC\xspace}

%% Chemical symbols
\def\cfourften     {\ensuremath{\mathrm{ C_4 F_{10}}}\xspace}
\def\cffour        {\ensuremath{\mathrm{ CF_4}}\xspace}
\def\cotwo         {\ensuremath{\mathrm{ CO_2}}\xspace} 
\def\csixffouteen  {\ensuremath{\mathrm{ C_6 F_{14}}}\xspace} 
\def\mgftwo     {\ensuremath{\mathrm{ Mg F_2}}\xspace} 
\def\siotwo     {\ensuremath{\mathrm{ SiO_2}}\xspace} 

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}\xspace}
\newcommand{\etal}{\mbox{\itshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}
%%% from the lifetime paper 

\def\bToJPsiX     {\decay{H_b}{\jpsi X}}
\def\BToJPsiX     {\decay{\B}{\jpsi X}}
\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}}
\def\BdToJPsiKstENT{\decay{\Bd}{\jpsi\KstarzENT}}
\def\BdToJPsiKS   {\decay{\Bd}{\jpsi\KS}}
\def\BuToJPsiK    {\decay{\Bu}{\jpsi K^+}}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}}
\def\LbToJPsiL    {\decay{\Lb}{\jpsi\Lz}}

\newcommand{\DOCAz}{\mbox{$\rho$}\xspace}









\def \btosll {\ensuremath {\bquark \to \squark \lepton^+\lepton^-}\xspace} 


\def \Pfive{$P^{\prime}_{5}$}

\def \Qfive{$Q^{\prime}_{5}$}



 
\def\Rll{\ensuremath{r_{\ell\ell}}\xspace}
\def\Rmm{\ensuremath{r_{\mm}}\xspace}
\def\Ree{\ensuremath{r_{\ee}}\xspace}
\def\RJPsi{\ensuremath{r_{\jpsi}}\xspace}
\def\invRJPsi{\ensuremath{r_{\jpsi}^{-1}}\xspace}
\def\RPsi{\ensuremath{R_{\psitwos}}\xspace}
\def\invRPsi{\ensuremath{R_{\psitwos}^{-1}}\xspace}

\def\RCC{\ensuremath{r_{\psitwos}}\xspace}
\def\RG{\ensuremath{r_{\gamma}}\xspace}
\def\RKst{\ensuremath{R_{\Kstarz}}\xspace}
\def\RK{\ensuremath{R_{\kaon}}\xspace}
\def\RpK{\ensuremath{R_{\proton\kaon}}\xspace}
\def\invRpK{\ensuremath{R_{\proton\kaon}^{-1}}\xspace}
\def\RH{\ensuremath{R_{H}}\xspace}
\def\RKK{\ensuremath{R_{\kaon^{(*)}}}\xspace}



==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash aleph} & \aleph & \texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal \\
\texttt{\textbackslash lthree} & \lthree & \texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash muon} & \muon \\
\texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb \\
\texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pizs} & \pizs & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson \\
\texttt{\textbackslash rhoz} & \rhoz & \texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom \\
\texttt{\textbackslash rhopm} & \rhopm & \texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb \\
\texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp \\
\texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp \\
\texttt{\textbackslash etaz} & \etaz & \texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz \\
\texttt{\textbackslash omegaz} & \omegaz &  \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash DorDbar} & \DorDbar \\
\texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz \\
\texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash Ds} & \Ds \\
\texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm \\
\texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp \\
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb \\
\texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp \\
\texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Lz} & \Lz \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar & \texttt{\textbackslash Lambdares} & \Lambdares \\
\texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar \\
\texttt{\textbackslash Sigmaresbarz} & \Sigmaresbarz & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Lc} & \Lc \\
\texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz \\
\texttt{\textbackslash Xibm} & \Xibm & \texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz \\
\texttt{\textbackslash Xibbarp} & \Xibbarp & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}


\def\myL {\ensuremath{\PLambda}\xspace}
\def\myLb {\ensuremath{\PLambda^0_\bquark}\xspace}
\def\myX {\ensuremath{\PXi^-}\xspace}
\def\myXst {\ensuremath{\PXi(1530)^0}\xspace}
\def\myXb {\ensuremath{\PXi^-_\bquark}\xspace}
\def\myO {\ensuremath{\POmega^-}\xspace}
\def\myOb {\ensuremath{\POmega^-_\bquark}\xspace}
\def\myXbz {\ensuremath{\PXi^0_\bquark}\xspace}
\def\myXcp {\ensuremath{\PXi^+_\cquark}\xspace}
\def\myXcz {\ensuremath{\PXi^0_\cquark}\xspace}
\def\jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb & \texttt{\textbackslash Vuds} & \Vuds \\
\texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds & \texttt{\textbackslash Vuss} & \Vuss \\
\texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss & \texttt{\textbackslash Vubs} & \Vubs \\
\texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt \\
\texttt{\textbackslash dpp} & \dpp & \texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> my-symbols-old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\def\qsqt{\ensuremath{q^{2}_{\textrm{true}}}\xspace}
\def\fqsqt{\ensuremath{\alpha_{\qsqt}}\xspace}
 
\def\lqsq{low-\qsq}
\def\cqsq{central-\qsq}
\def\hqsq{high-\qsq}
 
\def\pr{partially reconstructed }

\def\lomu{\texttt{L0Muon}\xspace}
\def\loel{\texttt{L0Electron}\xspace}
\def\lohad{\texttt{L0Hadron}\xspace}
\def\lotis{\texttt{L0Global\,(TIS)}\xspace}
\def\lotos{\texttt{L0Global\,(TOS)}\xspace}
 
\def\lom{\textrm{L0M}\xspace}
\def\loe{\textrm{L0E}\xspace}
\def\lol{\textrm{L0L}\xspace}
\def\loh{\textrm{L0H!}\xspace}
\def\loi{\textrm{L0I!}\xspace}
\def\lohi{\textrm{L0H}\xspace}
\def\loii{\textrm{L0I}\xspace}
\def\lotiis{\texttt{L0TIS}\xspace}
 
\def\tislh{\textrm{TIS1}\xspace}
\def\tosltish{\textrm{TIS2}\xspace}
 
\def\zg{\ensuremath{0\gamma}\xspace}
\def\og{\ensuremath{1\gamma}\xspace}
\def\tg{\ensuremath{2\gamma}\xspace}
 
\def\tap{\textrm{tag-and-probe}\xspace}
 
\def\tis{\textrm{TIS}\xspace}
\def\tos{\textrm{TOS}\xspace}
\def\tistos{\textrm{TISTOS}\xspace}
 
\def\kfold{\textit{k-fold}\xspace}
 
\def\splot{\ensuremath{_s\mathcal{P}lot}\xspace}
\def\splotted{\splot{\textrm{ted}}\xspace}
\def\sweight{\ensuremath{_s\mathcal{W}eight}\xspace}
 
\def\pidc{\texttt{PIDCalib}\xspace}
\def\loct{\texttt{L0CaloTool}\xspace}
 
\def\dtf{\texttt{DecayTreeFitter}\xspace}
\def\rkp{\texttt{RooKeysPdf}\xspace}
\def\bcat{\texttt{TupleToolMCBackgroundInfo}\xspace}
 
\def\nspd{\texttt{nSPDHits}\xspace}
 
\def\realet{\ensuremath{\texttt{real}^{\loct}_{E_{\textrm{T}}}}\xspace}
 
\def\KPi{\ensuremath{\Kp\pim}\xspace}
 
\def\mKpi{\ensuremath{m(\kaon\pion)}\xspace}
\def\mee{\ensuremath{m(\ee)}\xspace}
 
\def\mKpill{\ensuremath{m(\kaon\pion \ell\ell)}\xspace}
\def\mKpimm{\ensuremath{m(\kaon\pion \mm)}\xspace}
\def\mKpiee{\ensuremath{m(\kaon\pion \ee)}\xspace}
 
\def\mcKpill{\ensuremath{\mKpill_{\jpsi}}\xspace}
\def\mcKpimm{\ensuremath{\mKpimm_{\jpsi}}\xspace}
\def\mcKpiee{\ensuremath{\mKpiee_{\jpsi}}\xspace}
\def\mcpKpill{\ensuremath{\mKpill_{\psitwos}}\xspace}
\def\mcpKpimm{\ensuremath{\mKpimm_{\psitwos}}\xspace}
\def\mcpKpiee{\ensuremath{\mKpiee_{\psitwos}}\xspace}
 
\def\hop{\textsc{HOP}\xspace}
\def\mhop{\ensuremath{m(\kaon\pion \ee)_{\textrm{HOP}}}\xspace}
 
\def\wpid{\ensuremath{w_{\textrm{PID}}}\xspace}
\def\wmco{\ensuremath{w_{\textrm{Mult\&Kin}}}\xspace}
\def\wtrg{\ensuremath{w_{\textrm{Trg}}}\xspace}
\def\wlo{\ensuremath{w_{\textrm{\lone}}}\xspace}
\def\whlt{\ensuremath{w_{\textrm{\hlt}}}\xspace}
\def\wmct{\ensuremath{w_{\textrm{Data/MC}}}\xspace}
 
\def\etotal{\ensuremath{\varepsilon_{\textrm{tot}}}\xspace}
\def\egeom{\ensuremath{\varepsilon_{\textrm{geo}}}\xspace}
\def\ereco{\ensuremath{\varepsilon_{\textrm{rec}|\textrm{geo}}}\xspace}
\def\ePID{\ensuremath{\varepsilon_{\textrm{PID}|\textrm{rec}}}\xspace}
\def\etrig{\ensuremath{\varepsilon_{\textrm{trg}|\textrm{PID}}}\xspace}
\def\emva{\ensuremath{\varepsilon_{\textrm{MVA}|\textrm{trg}}}\xspace}
\def\ehop{\ensuremath{\varepsilon_{\textrm{\hop}|\textrm{MVA}}}\xspace}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%\def\leptonlepton{\ensuremath{\ellp\ellm}\xspace}
 
\def\bTosll{\decay{\bquark}{\squark \, \leptonlepton}}
\def\bTosmm{\decay{\bquark}{\squark \, \mm}}
\def\bTosee{\decay{\bquark}{\squark \, \ee}}
 
\def\pp{\ensuremath{\proton\proton}\xspace}
\def\mupm{\ensuremath{\mu^\pm}\xspace}
 
\def\mm{\ensuremath{\mu\mu}\xspace}
\def\ee{\ensuremath{ee}\xspace}
 
\def\Rll{\ensuremath{r_{\ell\ell}}\xspace}
\def\Rmm{\ensuremath{r_{\mm}}\xspace}
\def\Ree{\ensuremath{r_{\ee}}\xspace}
\def\RJPsi{\ensuremath{r_{\jpsi}}\xspace}
\def\RPsi{\ensuremath{r_{\psitwos}}\xspace}
\def\RCC{\ensuremath{R_{\psitwos}}\xspace}
\def\RG{\ensuremath{r_{\gamma}}\xspace}
\def\RKst{\ensuremath{R_{\Kstarz}}\xspace}
\def\RK{\ensuremath{R_{\kaon}}\xspace}
\def\RpK{\ensuremath{R_{\proton\kaon}}\xspace}
\def\RH{\ensuremath{R_{H}}\xspace}
\def\RKK{\ensuremath{R_{\kaon^{(*)}}}\xspace}
 
\def\KstKpi{\ensuremath{\Kstarz(\kaon\pion)}\xspace}
 
\def\JPsll{\ensuremath{\jpsi(\ell\ell)}\xspace}
\def\JPsmm{\ensuremath{\jpsi(\mm)}\xspace}
\def\JPsee{\ensuremath{\jpsi(\ee)}\xspace}
 
\def\Psill{\ensuremath{\psitwos(\ell\ell)}\xspace}
\def\Psimm{\ensuremath{\psitwos(\mm)}\xspace}
\def\Psiee{\ensuremath{\psitwos(\ee)}\xspace}
 
\def\Gee{\ensuremath{\gamma(\ee)}\xspace}
 
\def\Kone{\ensuremath{\kaon_{1}(1270)}\xspace}
\def\Ktwo{\ensuremath{\kaon_{2}^{*}(1430)}\xspace}

\def\Lst{\ensuremath{\Lambda^*}\xspace}
 
\def\BdToKstll{\decay{\Bd}{\Kstarz \leptonlepton}}
\def\BdToKstmm{\decay{\Bd}{\Kstarz \mumu}}
\def\BdToKstee{\decay{\Bd}{\Kstarz \epem}}
 
\def\BdToKststee{\decay{\Bd}{(\decay{X}{Y\Kstarz}) \epem}}
 
\def\BdToKstG{\decay{\Bd}{\Kstarz \gamma}}
\def\BdToKstGee{\decay{\Bd}{\Kstarz \gamma(\to\epem)}}
 
\def\BdToKstJPsi{\decay{\Bd}{\Kstarz \jpsi}}
\def\BdToKstKpiJPsill{\decay{\Bd}{\Kstarz(\decay{}{\kaon\pion}) \jpsi(\decay{}{\ell\ell})}}
\def\BdToKstJPsill{\decay{\Bd}{\Kstarz \jpsi(\decay{}{\leptonlepton})}}
\def\BdToKstJPsimm{\decay{\Bd}{\Kstarz \jpsi(\decay{}{\mumu})}}
\def\BdToKstJPisee{\decay{\Bd}{\Kstarz \jpsi(\to\epem)}}
 
\def\BdToXJPisll{\decay{\Bd}{X \jpsi(\decay{}{\leptonlepton})}}
\def\BdToXJPismm{\decay{\Bd}{X \jpsi(\decay{}{\mumu})}}
\def\BdToXJPisee{\decay{\Bd}{X \jpsi(\to\epem)}}
 
\def\BdToXPsiee{\decay{\Bd}{X \psitwos(\to\epem)}}
 
\def\BdToKstPsill{\decay{\Bd}{\Kstarz \psitwos(\to\leptonlepton)}}
\def\BdToKstPsimm{\decay{\Bd}{\Kstarz \psitwos(\to\mumu)}}
\def\BdToKstPsiee{\decay{\Bd}{\Kstarz \psitwos(\to\epem)}}
 
\def\BdToKststPsiee{\decay{\Bd}{(\decay{X}{Y\Kstarz}) \psitwos(\to\epem)}}
 
\def\BdToDll{\decay{\Bd}{\Dm(\to \Kstarz \ellm\nu) \ellp\nu}}
\def\BdToDl{\decay{\Bd}{\Dm\ellp\nu}}
\def\BdToDmm{\decay{\Bd}{\Dm(\to \Kstarz \mun\nu) \mup\nu}}
\def\BdToDee{\decay{\Bd}{\Dm(\to \Kstarz \en\nu) \ep\nu}}
\def\BdToDe{\decay{\Bd}{\Dm\ep\nu}}
 
\def\BdToKstEta{\decay{\Bd}{\Kstarz \eta}}
\def\BdToKstPiz{\decay{\Bd}{\Kstarz \piz}}
 
\def\BuToKll{\decay{\Bu}{\Kp \leptonlepton}}
\def\BuToKmm{\decay{\Bu}{\Kp \mumu}}
\def\BuToKee{\decay{\Bu}{\Kp \epem}}
 
\def\BuToKJPsill{\decay{\Bu}{\Kp \jpsi(\decay{}{\leptonlepton})}}
\def\BuToKJPsimm{\decay{\Bu}{\Kp \jpsi(\decay{}{\mumu})}}
\def\BuToKJPsiee{\decay{\Bu}{\Kp \jpsi(\to\epem)}}
\def\BuToKresoneee{\decay{\Bu}{\Kone^{+} \epem}}
\def\BuToKrestwoee{\decay{\Bu}{\Ktwo^{+} \epem}}
 
\def\BsToPhill{\decay{\Bs}{\phi\leptonlepton}}
\def\BsToPhimm{\decay{\Bs}{\phi\mm}}
\def\BsToPhiee{\decay{\Bs}{\phi\ee}}
\def\BsToKstJPsll{\decay{\Bs}{\Kstarz \jpsi(\decay{}{\leptonlepton})}}
\def\BsToKstJPsmm{\decay{\Bs}{\Kstarz \jpsi(\decay{}{\mumu})}}
\def\BsToKstJPsee{\decay{\Bs}{\Kstarz \jpsi(\decay{}{\ee})}}
\def\BsToKstPsill{\decay{\Bs}{\Kstarz \psitwos(\decay{}{\leptonlepton})}}
\def\BsToKstPsimm{\decay{\Bs}{\Kstarz \psitwos(\decay{}{\mumu})}}
\def\BsToKstPsiee{\decay{\Bs}{\Kstarz \psitwos(\decay{}{\ee})}}
 
\def\LbToLll{\decay{\Lb}{\Lz \leptonlepton}}
\def\LbToLmm{\decay{\Lb}{\Lz \mm}}
\def\LbToLee{\decay{\Lb}{\Lz \ee}}
\def\LbToLJPsill{\decay{\Lb}{\Lz \jpsi(\decay{}{\leptonlepton})}}
\def\LbToLG{\decay{\Lb}{\Lz \gamma}}
\def\LbToLGee{\decay{\Lb}{\Lz \gamma(\to\epem)}}
 
\def\LbTopKll{\decay{\Lb}{p\kaon \leptonlepton}}
\def\LbTopKmm{\decay{\Lb}{p\kaon \mumu}}
\def\LbTopKee{\decay{\Lb}{p\kaon \epem}}
\def\LbTopKJPsill{\decay{\Lb}{p\kaon \jpsi(\decay{}{\leptonlepton})}}
\def\LbTopKJPsi{\decay{\Lb}{p\kaon \jpsi}}
\def\LbTopKJPsimmee{\decay{\Lb}{p\kaon \jpsi(\decay{}{\mumu, \epem})}}
\def\LbTopKJPsimm{\decay{\Lb}{p\kaon \jpsi(\decay{}{\mumu})}}
\def\LbTopKJPsiee{\decay{\Lb}{p\kaon \jpsi(\to\epem)}}
\def\LbTopKPsill{\decay{\Lb}{p\kaon \psitwos(\decay{}{\leptonlepton})}}
\def\LbTopKPsimm{\decay{\Lb}{p\kaon \psitwos(\decay{}{\mumu})}}
\def\LbTopKPsiee{\decay{\Lb}{p\kaon \psitwos(\to\epem)}}
\def\LbTopKGee{\decay{\Lb}{p\kaon \gamma(\to\epem)}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%% for masses chapter 
\def\XibToXiJPsi{\decay{\Xi^-_b}{\jpsi} {\Xi^{-}}}
\def\OmegabToOJPsi{\decay{\Omega^-_b}{\jpsi} {\Omega^{-}}}

\newcommand{\chisqDTF}{\ensuremath{\chi^2_\mathrm{DTF}}\xspace}
\newcommand{\chisqIP}{\ensuremath{\chi^2_\mathrm{IP}}\xspace}

%\newcommand{\myXb} {\Xi_b^{-}}
%\newcommand{\myOb} {\Omega_b^{-}}


\def\myL{\ensuremath{\Lambda}\xspace}
\def\myLb{\ensuremath{\Lambda_b^{0}}\xspace}

\def\myXb{\ensuremath{\Xi_b^{-}}\xspace}
\def\myX{\ensuremath{\Xi^{-}}\xspace}

\def\myOb{\ensuremath{\Omega_b^{-}}\xspace}
\def\myO{\ensuremath{\Omega^{-}}\xspace}




==> papers.tex <==
% !TEX root = thesis.tex


\includepdf[pages={1,7,8,9,10,11,12,13,14,15}]{masses.pdf}
\includepdf[pages={1,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25,26,27,28,29}]{lifetimes.pdf}
\includepdf[pages={1,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22 }]{RpK.pdf}

==> theory.tex <==

\chapter{Allegro non troppo}

\epigraph{\textit {A Bird, came down the Walk - \\
He did not know I saw -\\ 
He bit an Angle Worm in halves \\
And ate the fellow, raw}}{Emily Dickinson}



\section{A powerful yet incomplete theory}
\label{sec:into} 
The Standard Model (SM) of particle physics was invented in the late 60's, it is a quantum gauge theory.
Similarly to a lego game, there are only a few different kinds of fundamental particles describing 
visible matter as we know it. The SM is structured in three families or generations of fermions
named quarks and leptons. There are six types of quarks {\it up, down, charm,  strange,  top} and {\it bottom}. 
The {\it bottom} quark (\bquark), is also referred to as $beauty$-quark. There are three  charged leptons  $e^{-},\mu^{-}, \tau^{-}$ and three associated neutral leptons $\nu_{e},\nu_{\mu}, \nu_{\tau}$~\cite{PDG}. 
By construction in the SM,  three interactions  {\it i.e.}: the electromagnetic, weak and strong interactions are responsible for the transitions between these particles.  These interactions are mediated by particles called gauge bosons, \g,  \Z and \W, the gluons, they are described by a gauge group $SU(3)_c\times SU(2)_{L}\times U(1)_{Y}$. 
This group is spontaneously  broken down to $SU(3)_c\times U(1)_{em}$, $i.e:$ QCD and QED, through the non-vanishing vacuum expectation value of the Higgs field.
Depending on the  properties of the fermions and bosons at play,  such as electric charge and other quantum numbers,  particles will be affected by the interactions in different ways. For example, given that they carry a charge of ``colour" only quarks are affected by the strong interaction.  
The SM of particles physics  has often been described as an elegant theory; this is partly due to its precise predictive power. The SM is also appealing since it offers a wide class of physics observables that can be confronted with experimental measurements, a few  examples of which will be discussed in this habilitation. 
This being said, the SM fails to describe some fairly fundamental aspects of nature. 
The SM does not accommodate gravity, nor can it explain the mass hierarchy of many orders of magnitude observed between particles. For instance, the mass of an electron is 0.511 MeV/$c^2$ and the mass of the top quark is 173 GeV/$c^2$~\cite{PDG}.  Furthermore, satellite experiments such as Planck show that visible matter only comprises 5 \% of the universe, the rest  is attributed to dark energy (68\%) and dark matter (27 \%)~\cite{Planck}.
In other words, the SM is excellent at describing what seems to be the tip of an iceberg. 
Both the theory and experimental physics communities share the viewpoint that there must exist sources of New Physics (NP), new theories able to propose a more complete description of nature. 

One of the main purposes of  the experiments located at the Large Hadron Collider at CERN, is to search for new particles. 
Experimentally, there are two strategies to search for these unknown particles.  The first approach is to ``hunt" directly for new particles in the decay products of the proton-proton collisions. This is how the Higgs boson  was discovered in 2012 by the ATLAS and CMS collaborations~\cite{Higgs}. 
A second approach  is to demonstrate the presence of  new particles in an indirect way.  The heart of indirect searches relies on a  class of physics observables  that may differ from  SM predictions in the presence of NP.  This method is heavily exploited by the LHCb experiment.  If one assumes that NP lies at a scale $\Lambda_{\textrm{NP}}$ higher than the mass of the weak interaction bosons, then one can write a Lagrangian as follows: 
\begin{equation}
{\cal L}_{ \textrm { \tiny NP}} = {\cal L}_{\textrm{ \tiny SM}} +   \sum_{d>4}   \sum_{n=1}^{N_d} \frac{c_{n}^{(d)}}{\Lambda_{\textrm{\tiny NP}}^{d-4}} {\cal O}_n^{ (d)}, 
\label{eq:lagrangian}
\end{equation}
where the NP is described by higher order operators suppressed by a scale $\Lambda_\textrm {NP}$.  The rule of  the game of flavour physics is twofold. On the one hand  it is essential to understand and constrain as precisely as possible SM processes, where no NP is expected. These class of processes are sometimes called ``standard candles", they can be probed using dedicated observables such as mass or lifetime measurements. The second aspect is to search for deviations from SM predictions using ``theoretically clean" probes, for instance angular observables, lepton universality tests, \etc 

This chapter is organised as follow, after a discussion of the theoretical framework employed to make predictions,  three  observables, namely, masses, lifetimes, and lepton universality tests be will described.  They serve as illustrations of how one can poke at different aspects of the physics that we care about.  
%-----
%-----
%-----
%-----
%\section {Un fil conducteur}
As will be later discussed in Chapter 2 and 3, the LHCb detector is specialised in the analysis of decays of hadrons containing a \bquark-quark. Following the hadronisation  which occurs after the production of pairs of \bquark-quarks (for instance in gluon-gluon fusion processes) all types of \bquark-hadrons are produced and in particular \bquark-baryons.  Their organisation within a quark model is shown in Figure~\ref{fig:quarkmodel}.  \bquark-baryons have emerged as a pattern in the research that I have conducted in the past years.  Their properties and the observables that they allow to reach are used as a ``fil conducteur" throughout the work documented in this habilitation.
%have a look at the expectations of Heavy Quark Symmetry. 
%
\begin{figure}[h]
\centering
\includegraphics[width=0.75\textwidth] {figs/theory/multiplets.png}%
\caption{\small SU(4) multiplets of baryons made of \uquark, \dquark, \squark and \bquark quarks. Left: the multiplet with an SU(3) octet on the lowest level. Right: the multiplet with an SU(3) decuplet on the lowest level. Observed states are shown in red, while predicted unobserved states are in blue~\cite{PDG}.}
\label{fig:quarkmodel}
\end{figure}
\section{Handling multi-scale problems}
Effective Field Theories (EFTs) are powerful tools to describe high energy NP phenomena and their effect on precision observables. Their strength lies in their ability to separate and treat multi-scale problems such as for example \bsll transitions.  At each scale, all the degrees of freedom with properties higher than the value of the scale will be integrated out. For instance,  let us consider tree-level   \bquark\to\cquark decay, in the SM  at the lowest order  it mediated by the exchange of \W boson, these transitions are referred to  a Flavour Changing Charged Current (FCCC). 
For this type of decay, the momentum transfer from the \W is very small in comparison to its mass, one can write: 
\begin{equation}
\frac{-g_{\mu\nu} + q_\mu q_\nu/M_\W^{2}}{q^{2} - M_\W^{2}} \xrightarrow[]{q^2 \ll M_\W^{2}} \frac{g_{\mu\nu}}{M_\W^{2}},
\end{equation}
The charged current can be reduced to a point-like four fermion interaction by "integrating-out" the \W boson. This is illustrated  in Figure:~\ref{fig:fermi}.
%--%%%
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth] {figs/theory/fermi.png}%
\caption{\small Example of "integrating-out" a $W$ boson in a FCCC.}
\label{fig:fermi}
\end{figure}
%%%%%%
%%%%%%
Different models can be adopted depending on the scale where one is trying to address a specific problem or make a prediction for a physics observable. Examples of models which will be later discussed in this document as a function of energy are illustrated in Figure~\ref{fig:EFT}. What makes EFTs powerful to describe NP is that they can be used to study processes, where one does not know a priori the underlying ultra violet (UV) theory~\cite{Fuentes-Martin:2019mun,Becirevic:2018afm}. 
Another  usage of EFT  is the study of low energy properties of the strong interaction, for example Chiral Perturbative Theory or Heavy Quark Expansion Theory~\cite{Pich:1998xt,Neubert:1996wg} which do not  rely on fully perturbative computations. 

%%%%%%
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth] {figs/theory/EFT_UV.png}%
\caption{\small Sketch of relevant energy scale (first line), New Physics ETFs and QCD ones.  }
\label{fig:EFT}
\end{figure}
%%%%%%

In the EFT framework, the phenomenology of \bquark-decays can be described in a convenient way,  with an Effective Hamiltonian formalism~\cite{Pich:1998xt, Buras:1998raa, Silvestrini:2019sey}.  For a given initial state $I$ going to a final state $F$, the amplitude can be written as :
%---%%%%
\begin{equation}
{\cal A} (I \to F )=    \bra  F  {\cal H}_{\textrm{eff}}  \ket I, 
\end{equation}
%%%%%%
where the $ {\cal H}_{\textrm{eff}} $ describes both the low energy dynamics (long distance) and high energy ones (short distance).  
%%%%%%
%\begin{equation}
% {\cal H}_{\textrm{eff}} = \textrm {constants} \times  \textrm {long distance }\times \textrm {short distance}
%\end{equation}
%%%%
%---
%In this formalism, the low energy dynamic does not depend on the high energy one. 
%Once, an energy $E$ scale is selected to treat the important physics effects, large energy gaps are put to zero (infinity) the light (heavy). These energy scales are represented by  $m$ and $M$ respectively:
%\begin{equation}
%0 \leftarrow m  \ll  E  \ll   M \rightarrow \infty
%\end{equation}
 %Finally, the only remnants of the high-energy dynamics are in the low-energy couplings and in the symmetries of the EFT.


\section{What can we learn from mass measurements?}
A hadron can be thought of as a bound state of constituent quarks. It can either form a meson ($q\bar{q}$), a baryon ($qqq$, $\bar{q}\bar{q}\bar{q}$) or more exotic combinations such as tetra- or pentaquarks~\cite{PDG2018}. This classification was first proposed by Gell-Mann and Nishijima in 1958.  The generalised Gell-Mann-Nishijima formula relating the various hadron quantum numbers is given by:
\begin{equation}
Q = I_{z} + \frac{ {\cal B } + S + C + B + T }{2}
\label{eq:gell}
\end{equation}
where $Q$ is the charge, $\cal{B}$ is the baryon number, $I_{z}$ is the $z$ projection of the Isopsin and $S,C,B$ and $T$ are the {\it flavour} of the quark. While, we know today that there are six types of quarks, {\it up, down, strange, charm, top} and {\it beauty}, one should remember that at that time, Gell-Mann and Nishijima, nor any other physicists, were not aware of the existence of neither the  {\it charm, beauty} nor the {\it top} quark. Nevertheless, they were able to predict the existence of the $\Omega^{-}$({\it{sss}}) baryon discovered in 1964 in a hydrogen bubble chamber.
 %from hep-lat/99120342v2. 
The masses, which are one of the most fundamental properties of all hadrons, are a pure QCD effect. One could write in a simplified way: 
\begin{equation}
m_{\textrm {hadron}} = \sum_{i}  m^{i}_{\textrm {quark}}  +  E_{\textrm{Binding}}
\end{equation}
%The notion of quark masses is slightly ambiguous, except for the top quark, there are no free quarks in nature, .
 Except for the top quark, there are not free quarks in nature. This makes the information about their mass difficult to access. Furthermore, the binding energy is completely driven by QCD effects. Therefore,  relatively large uncertainties in the theoretical description of hadron masses are expected, see for example those predictions listed in Table~\ref{tab:predictions}.
Given that baryons are three-body systems, the theory describing their dynamics within quark models is much more complicated than that for mesons. 
There are many approaches used within QCD to predict their properties.  For example non-relativistic formulations of QCD, quark models~\cite{PDG} or light-cone sum rules~\cite{Colangelo:2000dp}  allow us to investigate the dependence of  the baryon mass splittings on the heavy and light quark masses.  In lattice QCD, the correlation functions used to compute the action for baryons are more difficult to determine than those for mesons, therefore it is comparatively harder to extract a reliable mass spectrum for heavy baryons~\cite{Mathur:2002ce}.
The predictions of the CQM~\cite{Karliner:2009} method for example, rely on the knowledge of the charm baryonic counter part.
The spread of the predictions and their uncertainties in Table~\ref{tab:predictions} demonstrate that precise measurements of many heavy hadron and in particular \bquark-baryon  masses help to either exclude some of the theoretical approaches or  contribute to refining them. Furthermore, a better understanding of the dynamics of quarks inside the hadrons  can help to understand and characterize  the nature of exotic particles, such as the pentaquarks, the $X(3872)$ or the $Z(4140)$, \etc which have been observed in the past years at the $B$-factories and at the LHC~\cite{PDG}.

\begin{table}[h]
\centering
\begin{tabular}{l | c | c |c }
Prediction & \Lb mass & \Xibm mass & \Omegab mass \\
\hline 
CQM~\cite{Karliner:2009} & Used as input & 5790-5800 & 6052.1 $\pm$ 5.6\\
$1/N_c$  expansion~\cite{Jenkins:2007dm}  & Used as input & Used as input  & 6039.1 $\pm$ 8.3 \\
RCQM~\cite{Ebert:2005xj}& 5211$\pm$ 100 & 5812 $\pm$ 100 & 6065 $\pm$ 100\\
HQET + QCD sum rule~\cite{Liu:2007fg}  &$  5637^{+68}_{-56}$ &$ 5780^{+73}_{-68}$ & $6036 \pm 81$ \\
QCD sum rule~\cite{Zhang:2008rm} &$ 5690 \pm 130$ & & $5890 \pm 180$ \\
Lattice QCD~\cite{Lewis:2009ce}&$ 5641 \pm 21 ^{+15}_{-33}$ &$ 5781 \pm 17^{+17}_{-16} $& $6006 \pm 10 ^{+20}_{-19}$ \\
\end{tabular}
\caption{\small Mass predictions in \mevcc for \Lb, \Xibm and \Omegab baryons.}
\label{tab:predictions}
\end{table}



%----
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----
\section{What can we learn from lifetime measurements?}
Another fundamental property of particles is their lifetime. While at first order all \bquark-hadron lifetimes are expected to be the same, 
the presence of the spectator quark displayed in Figure~\ref{fig:tree} can not be ignored in accurate numerical computations. Non-perturbative effects to heavy-flavour decays can be expressed through an expansion in inverse powers of $m_{\bquark}$. 
The decay rate of the transition of a \bquark-hadron, $H_{\bquark}$, to an inclusive final state $X$, can be expressed in terms of a phase-space integral (PS) of 
the square of the matrix element, summed over all final state $X$ with the same quantum numbers
\begin{equation}
\Gamma (H_\bquark \to X) =  \frac{1}{2m_{H_{\bquark}}} \sum_{X} \int_{\textrm{PS}} (2\pi)^{4} \delta^{(4)} ( p_{H_{\bquark}} - p_{X}) | \bra X  H_{\textrm {eff}}  \ket  {H_{\bquark}} |^{2}
 \end{equation}
Explicitly calculating the integral, one arrives at the Heavy Quark Expansion~\cite{Neubert:1996wg} of decay rates of heavy hadrons:
\begin{equation}
\Gamma  (H_\bquark \to X)  =   \Gamma_{0} + \frac {\Lambda^{2}}{m_{\bquark}^{2}} \Gamma_{2}  +  \frac {\Lambda^{3}}{m_{\bquark}^{3}}  \Gamma_{3} +   \frac {\Lambda^{4}}{m_{\bquark}^{4}}\Gamma_{4} + ...,
\end{equation}
where the expansion parameter is denoted ${\Lambda}/{m_{\bquark}}$, where the typical scale of $\Lambda$ is $\sim$ 1 GeV. 

Each of the $\Gamma_i$ terms of the expansion describes different aspects of the possible effects inside the hadrons. 
\begin{itemize}
\item  $\Gamma_{0}$ {\it spectator model} all $b$-hadrons have the same lifetime.
\item There are no corrections in $1/m_\bquark$. 
\item  $\Gamma_{2}$   {\it Fermi motion} and {\it chromomagnetic interaction}, first corrections due to the strong interaction, isospin, at this order one would expect : 
$\tau_\Bu/\tau_\Bz -1 \approx 0$ and $\tau_\Lb/\tau_\Bz -1 \approx 2\%$.
\item  $\Gamma_{3}$  {\it Weak annihilation} and {\it Pauli interference}, the spectator quark is involved only at  $1/{m_{\bquark}^{3}}$ order.
\end{itemize}
The measurement of the lifetime differences of \bquark-hadrons allows therefore to test HQET at the third order.
\begin{figure}[h]
\centering
\includegraphics[width=0.7\textwidth] {figs/theory/tree-levelJpsiLambda.png}%
\caption{\small Feynman diagram of $\Lb\to \jpsi\Lz^{(*)}$}
\label{fig:tree}
\end{figure}


%Can make a few comments here. 
One important assumption behind the heavy quark expansion is the so-called {\it quark-hadron} duality. It can be translated as follows: rates computed at the quark-gluon level  are equal to the corresponding  observables involving hadrons. Extensive discussions can be found in the literature regarding this assumption. 
One of the best ways to test this is to confront HQET computations to experimental measurements. 
A detailed review and summary of HQET principles can be found in Ref.~\cite{Lenz:2015dra} and useful references can be found in Refs.~\cite{Bigi:1995jr},\cite{Cheng:1997xba}, \cite{Ito:1997qq}.

%------------------------
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----
\section{What can we learn from Lepton Universality tests?}
\label{sec:LU}

%------------------------
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----
%----%----%----%----%----%----%----

Within the SM, there are no Flavour Changing Neutral Currents (FCNC) at tree level, as a consequence  \bsll transitions can only occur through loops. 
%, these are processes in the SM. 
Therefore, NP contributions can compete with the SM ones, which makes \bsll transitions a particularly  interesting laboratory.  For instance, in Figure:~\ref{fig:b2sll-ex} the SM gauge boson $Z$ could be replaced by a  new particle,  such as a heavier gauge boson, for example the  $Z^{\prime}$ or Leptoquarks. 
%These new phenomena are often predicted to appear at large energy scales of the order of the  TeV.  Therefore, Wilson coefficients can be modified by the presence  of these new phenomena or through new operators in the effective Hamiltonian that arise from sources
%beyond the SM.

 %Hence, they be seen as probes to test the existence of  NP at certain energy scales.   This is a typical example of an indirect search of new particles. 
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth] {figs/theory/b2sll-ex.png}%
\caption{\small Feynman diagram of a \bsll transition. }
\label{fig:b2sll-ex}
\end{figure}

For these decays, the effective Hamiltonian,  ${\cal H}_{\textrm{eff}}$ is defined as: 
\begin{equation}
{\cal H}_{\textrm{eff}} = \frac{G_F}{\sqrt{2}}\lambda^{\textrm{CKM}}\sum_{i} C_i{\cal O}_i,
\label{eq:EH}
\end{equation}
where $G_F$ is the Fermi constant and $\lambda^{\textrm {CKM}}$ are the Cabibbo-Kobayashi-Maskawa  terms describing the coupling between the $W^{\pm}$ bosons and the quarks~\cite{PDG}. 
In this formalism, the hard contributions generated by the electromagnetic, weak, and strong interactions can be factorised depending on their energy scale at leading order.
The low energy part of the transition,  typically lower than  the mass of the $b$-quark,  mediated for example by soft gluons,  is encoded  in what are called hadronic matrix elements, ${\cal O}_i$.
These elements can be evaluated using ``numerical" techniques such as Lattice QCD~\cite{Lattice}.
The Wilson coefficients $C_i$, on the other hand describe short distance contributions to the transition occurring at high energy, typically $\cal{O}$($m_W$). These coefficients can be calculated using perturbative methods~\cite{Wilson}. 

As shown in Equation~\ref{eq:EH}, with EFTs one can factorise long distance from short distance components. 
The short distances parts, which are sensitive to NP, are encoded in the Wilson coefficients. The dominant operators  relevant for \bsll transitions are: 
\begin{equation}
{\cal O}_7 = \frac{e}{16\pi^{2}} m_{\bquark} (\bar{s}\sigma_{\mu\nu} P_R \bquark) F^{\mu\nu} ;
\end{equation}
\begin{equation}
{\cal O}_9 = \frac{e^{2}}{16\pi^{2}}  (\bar{s}\gamma_{\mu} P_L \bquark)  (\bar{\lepton}\gamma^{\mu} \lepton);
\end{equation}
\begin{equation}
{\cal O}_{10} = \frac{e^{2}}{16\pi^{2}} (\bar{s}\gamma_{\mu} P_L \bquark)  (\bar{\lepton}\gamma^{\mu} \gamma_{5} \lepton);
\end{equation}
where $P_{L,R} = (1 \mp \gamma_5)/2$ are the projectors for left-(right-)handed chirality. $P_L$ corresponds to the $V-A$ structure of the weak interaction in the SM.
Due to the universality of lepton couplings for the three generations, the SM Wilson coefficients have the same value for all three lepton generations.  The determination of the Wilson coefficients requires a matching of the high-energy theory (in this case the SM) and at the electroweak scale and a running from this scale down to the low-energy one close to the mass of the \bquark quark. 
NP can manifest itself as shifts to the Wilson coefficients or enhancements of new operators which are either absent or strongly suppressed in  the SM.  

\noindent
One interesting feature of  \btosll decays is shown in Figure:~\ref{fig:q2}. It displays the variation of the differential rate \ie  the probability of a \btosll decay  to occur as a function of $q^2$, where $q^2$ is the sum square of the di-lepton system invariant mass. 
In particular, it is worth  noting that Wilson coefficients ($C_7^{(\prime)}, C_9^{(\prime)}, C_{10}^{(\prime)}$)   contribute differently to the different $q^2$ regions.  For example, the very low $q^2$ region is dominated by the Wilson coefficient $C_7^{(\prime)}$ corresponding to a Feynman diagram where a photon is produced as illustrated in Figure:~\ref{fig:q2}. Therefore, to fully exploit the rich phenomenology of these decays,  experimental measurements, such as branching fractions, forward-backward asymmetry, \etc are performed as a function of \qsq.
\begin{figure}[h]
\centering
\includegraphics[scale=0.4]{figs/theory/qsquare.pdf}
\caption{Differential rate as a function of \qsq in \bsll transitions.}
\label{fig:q2}
\end{figure}
%---
In order to constrain the values of the Wilson coefficients, the LHCb collaboration has conducted many measurements of \bsll transitions, such as differential branching fraction of \BuToKmm, \BdToKstmm, as well as $\Bs\to\phi\mu^{+}\mu^{-}$ and $\Lb \to \Lz \mu^{+}\mu^{-}$. A few deviations have been observed with respect to the SM predictions. 
Similar patterns have been observed in angular analyses, where optimised observables, for example \Pfive~, have been designed and employed to minimize the impact of hadronic uncertainties, as shown in Figure:~\ref{fig:p5}. 
\begin{figure}[h]
\centering
\includegraphics[width=0.55\textwidth] {figs/theory/p5.png}%
\caption{\small Measurements of \Pfive~ by different experiments, compared to the theoretical predictions.}
\label{fig:p5}
\end{figure}
%-----

%-----
Lepton Universality (LU)  is an ``accidental" property of the SM. It predicts equal coupling of the SM gauge bosons to all three families of leptons at tree-level. 
Lepton universality tests form some of the ``cleanest" observables, since all the hadronic uncertainties in these decays cancel in the ratios leaving only differences due to QED corrections, which are expected to be very small~\cite{SMPredIsidori}.  This property can be tested in many sectors and in particular in loop-induced  decays such as \btosll transitions, but also tree-level decays such as $\bquark \to \cquark \ell \nu_{\ell}$ decays. For this latter process, the ratios  $\RD = 0.299~\pm~ 0.003 $  and  $\RDst =0.258~ \pm~ 0.005 $ were measured at the $B$-factories and LHCb and lie 3.5 standard deviations above the SM predictions. The current world average agrees with the SM at only three standard deviations~\cite{Amhis:2019ckw}.
 For \btosll transitions, the LU ratios are defined as as: 
\begin{eqnarray}
\RH \equiv \frac{\bigintssss \frac{ d\Gamma(B \to H \mumu) }{d\qsq} \, d\qsq}{\bigintssss \frac{ d\Gamma(B \to H\epem) }{d\qsq} \, d\qsq} \, .
\end{eqnarray}
%-----
%-----
LU in \bsll decays has been tested until now in $B$ meson decays by the LHCb experiment~\cite{Aaij:2019wad}, \cite{Rkst},  and the results as a function of \qsq are :
\begin{equation}
\RK = 0.846 ^{ +0.060}_{ -0.054}   \mbox{ }^{+0.016}_{-0.014},  \mbox{ } \qsq \in [1, 6] \gevgevcccc,
\end{equation}
$$
\RKst = \left\{ 
		\begin{array} {ll}   
		0.66 ^{ +0.11}_{ -0.07}   \pm 0.03, \mbox{ } \qsq \in [0.045, 1.1] \gevgevcccc, \\ 
		 0.69 ^{ +0.11}_{ -0.07}   \pm 0.05,  \mbox{ } \qsq \in [1.1, 6.0] \gevgevcccc.
		 \end{array}
 \right.
 $$
 While these results are still statistically limited, it is important to extend the scope of these measurements to verify if the pattern of a ``deficit" of muons emerging from the LU tests together with the branching fraction measurements in the muonic decays~\cite{Aaij:2015esa,Aaij:2014pli},  holds or not. 
 
Recently, Ref.\cite{Fuentes-Martin:2019mun} argued that if NP has a $V-A$ structure, \ie $C_9 = -C_{10}$, then one expects in the SM that the electron-muon LU ratios across all species of \bquark-hadrons should be the same:  
%--------
\begin{equation}
\RK \approx  \RKst   \approx  R_{K\pi\pi}  \approx  R_{K_S} \approx  R_{\phi}   \approx   R_{\Lambda}  \approx  \RpK. 
\end{equation}
The first test of lepton universality with a \bquark-baryon is discussed in this habilitation in Chapter 3. 
%
%
%\section {Global fits and New Physics models}
%\section {What is emerging ?}
\section {What is emerging in the Loch Ness?}
\label{sec:usualsuspects}
As of today there are a few phenomenological attempts to fits the Wilson coefficients.  While some of these approaches differ in their treatment of the hadronic uncertainties~\cite{Ciuchini:2018anp}, which can manifest themselves in the size of the uncertainties on form factors for instance, most of them seem to draw a similar picture. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.40\textwidth]{figs/theory/C9-postMoriond.png}
\caption{Likelihood contours from neutral current LFU observables and the global fit in the the plane of a lepton flavour universal contribution to $C_9^{\textrm {univ}}$ Figure taken from Ref.\cite{Aebischer:2019mlg}.}
\label{fig:c9moriond}
\end{figure}

An example of such a phenomenological study~\cite{Aebischer:2019mlg} is shown in Figure~\ref{fig:c9moriond}.   The selected result  displays one of the phenomenological global fits, with a  lepton flavour universal  $C_9^{\textrm {univ}}$ Wilson coefficient shown as a function of  a scenario linking a purely muonic contribution to $C_{9}$ and a $C_9^{~bs\mu\mu} = - C_{10}^{~bs\mu\mu} $ hypothesis,   before and after the inclusion of the latest  \RK result from LHCb.  This pattern of Wilson coefficients  can be found in several NP  models with tree-level mediators, such as Leptoquarks.

While there has been  a myriad of theory developments in the past few years to interpret the flavour anomalies in a consistent and coherent way,  Leptoquarks, which are tree-level mediators, have received particular attention.  Given the experimental constraints from both loop-induced currents and tree-level decays, there are today three viable options for Leptoquarks models summarised in Table~\ref{tab:LQ}. The first option is based on models which predict a  $U_1$ Leptoquark and necessitate UV completion~\cite{DiLuzio:2017vat,  Calibbi:2017qbu, Bordone:2017bld, Barbieri:2017tuq}.  The other two make use of  two scalar Leptoquarks $S_1+S_3$ \cite{Crivellin:2017zlb, Buttazzo:2017ixm, Marzocca:2018} or $S_3 + R_2$ \cite{Becirevic:2018afm}. It will be most interesting to see in the next few years which scenarios survive the additional experimental constrains. 
\begin{table}[h]
\centering
\begin{tabular}{l  |c |  c | c }
Model & $R_{K^{(*)}}$ 	& $R_{D^{(*)}}$ & $R_{K^{(*)}}$ \&  $R_{D^{(*)}}$\\
&& &\\
\hline 

	$S_1= (3,1)_{-1/3}$	 &  \ding{54}  &\ding{52} &  \ding{54}  \\ 
	$R_2= (3,2)_{~7/6}$	 &  \ding{54}  &\ding{52} &  \ding{54} \\
	$\widetilde{R}_2= (3,2)_{~1/6}$	 &  \ding{54}  &\ding{54} &  \ding{54} \\
        $S_3= (3,3)_{-1/3}$	 &  \ding{52}  &\ding{54} &  \ding{54} \\
	$U_1= (3,1)_{~2/3}$	 &  \ding{52}  &\ding{52} &  \ding{52}\\
	$U_3= (3,3)_{~2/3}$	 &  \ding{52}  &\ding{54} &  \ding{54} \\
\end{tabular}
\caption{Summary of Leptoquark models which can accommodate  $R_{K^{(*)}}$ , $R_{D^{(*)}}$  and both. Table based work from  Ref.~\cite{Angelescu:2018tyl}. The SM quantum numbers are denoted by $(SU(3)_{c}, SU(2)_L)_Y$. }
\label{tab:LQ}
\end{table}

Pick your horse in Figure~\ref{fig:NP}, the bets are open ! 

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth] {figs/theory/NP.png}%
\caption{\small Example of NP Feynman diagrams~\cite{Romao:2017qnu},\cite{BecirevicLQ},\cite{Arnan:2019uhr}.}
\label{fig:NP}
\end{figure}


%
%
%
%
%
%
%
%
%






==> tikzfeynman.keys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynman@cs@angle@step{30}
      \def\tikzfeynman@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynman@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynman@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynman@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynman@cs@points@per@step,
    switch if less than=1.25*\tikzfeynman@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynman@cs@current@angle+\tikzfeynman@cs@angle@step, 360)}
      \let\tikzfeynman@cs@current@angle=\pgfmathresult%
    },
  ]{
    \pgfmathparse{sin(\tikzfeynman@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzfeynmanset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynman/.code={},
  execute at end feynman/.code={},
  every feynman/.style={/tikzfeynman/every feynman@@/.append style={#1}},
  every feynman@@/.style={
    /tikzfeynman/.cd,
    /tikzfeynman/medium,
  },
  execute at begin feynman@@/.code={}                     %% Internal version
  execute at end feynman@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Diagrams
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every diagram/.style={/tikzfeynman/every diagram@@/.append style={#1}},
  every diagram@@/.style={
    /tikzfeynman/.cd,
    .search also={/tikz/graphs, /tikz},
    nodes={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every vertex@@,
      /tikzfeynman/every vertex},
    edges={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every edge@@,
      /tikzfeynman/every edge},
    /tikzfeynman/medium,
  },
  every inline/.style={/tikzfeynman/inline@@/.append style={#1}},
  every inline@@/.style={
    /tikzfeynman/small,
  },
  inline/.style={
    /tikz/baseline={#1},
    /tikzfeynman/every inline@@,
  },
  every small/.style={/tikzfeynman/small@@/.append style={#1}},
  every small@@/.style={
    /tikz/node distance=1cm,
    /graph drawing/node distance=1.25cm,
    /graph drawing/level distance=1cm,
    /graph drawing/sibling distance=1.5cm,
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=1mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=0.5cm},
    /tikzfeynman/arrow size=1.2pt,
    /tikzfeynman/insertion/size=2.5pt,
  },
  small/.style={/tikzfeynman/every small@@},
  every medium/.style={/tikzfeynman/medium@@/.append style={#1}},
  every medium@@/.style={
    /tikz/node distance=1.5cm,
    /graph drawing/node distance=1.9cm,
    /graph drawing/level distance=1.5cm,
    /graph drawing/sibling distance=2.25cm,
  },
  medium/.style={/tikzfeynman/every medium@@},
  every large/.style={/tikzfeynman/large@@/.append style={#1}},
  every large@@/.style={
    /tikz/node distance=2cm,
    /graph drawing/node distance=2.5cm,
    /graph drawing/level distance=2cm,
    /graph drawing/sibling distance=3cm,
    /tikz/graphs/edges={thick},
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=4mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=1cm},
    /tikzfeynman/arrow size=1.6pt,
    /tikzfeynman/insertion/size=4pt,
  },
  large/.style={/tikzfeynman/every large@@},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynman/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynman/every vertex@@,
  },
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=1.5mm,
  },
  every dot/.style={/tikzfeynman/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynman/every dot@@,
  },
  every square dot@@/.style={
    /tikz/shape=rectangle,
  },
  every square dot/.style={/tikzfeynman/every square dot@@/.append style={#1}},
  square dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every square dot@@,
  },
  every empty dot@@/.style={
    /tikz/fill=none,
  },
  every empty dot/.style={/tikzfeynman/every empty dot@@/.append style={#1}},
  empty dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every empty dot@@,
  },
  every crossed dot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=3mm,
  },
  every crossed dot/.style={/tikzfeynman/every crossed dot@@/.append style={#1}},
  crossed dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every crossed dot@@,
  },
  every blob@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill=none,
    /tikz/outer sep=0.5\pgflinewidth,
    /tikz/inner sep=0pt,
    /tikz/minimum size=0.75cm,
    /tikz/pattern=north west lines,
  },
  every blob/.style={/tikzfeynman/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynman/every blob@@,
  },
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep=0.5\pgflinewidth,
  },
  every particle/.style={/tikzfeynman/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynman/every particle@@,
    /tikz/graphs/as={#1},
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynman@arrow@size,
  arrow size=1.5pt,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          rotate=180,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynman/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw
    },
  },
  every plain/.style={/tikzfeynman/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynman/every plain@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynman/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynman/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynman/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynman/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynman/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynman/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynman/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynman/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
    },
  },
  every scalar/.style={/tikzfeynman/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynman/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynman/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynman/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/thick,
    },
  },
  every ghost/.style={/tikzfeynman/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynman/every ghost@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynman/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynman/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynman/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynman/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.33,
      /tikzfeynman/with reversed arrow=0.73,
    },
  },
  every majorana/.style={/tikzfeynman/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynman/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.33,
      /tikzfeynman/with arrow=0.73,
    },
  },
  every anti majorana/.style={/tikzfeynman/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynman/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        coil,
        aspect=0.75,
        mirror,
        segment length=1.5mm
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynman/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynman/every gluon@@,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynman,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynman@insertion@size,
  insertion/size=3pt,
  insertion/style/.store in=\tikzfeynman@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynmanset{insertion/.cd,#1}
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, \tikzfeynman@insertion@size);
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, \tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynman,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynman@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynman@momentum@arrow@distance,
  momentum/arrow distance=3mm,
  momentum/arrow shorten/.store in=\tikzfeynman@momentum@arrow@shorten,
  momentum/arrow shorten=0.15,
  momentum/label style/.store in=\tikzfeynman@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynman@momentum@arrow@style,
  momentum/arrow style={},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
    /tikz/looseness=1.5,
  },
  half right/.style={
    /tikz/bend right=90,
    /tikz/looseness=1.5,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graceful Failure of LuaTeX keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@luatex@required@path{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath/\pgfkeyscurrentname' requires LuaTeX.  It will be ignored.}
}
\def\tikzfeynman@luatex@required@key{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath' requires LuaTeX.  It will be ignored.}
}

\ifluatex\else
  \pgfkeys{
    /graph drawing/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/graphs/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/horizontal/.code=\tikzfeynman@luatex@required@key,
    /tikz/horizontal'/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical'/.code=\tikzfeynman@luatex@required@key,
    /tikz/tree layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/layered layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring electrical layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/electric charge/.code=\tikzfeynman@luatex@required@key,
  }
  % \tikzfeynmanset{
  %   horizontal/.code={The key 'horizontal' requires LuaTeX.  It will be ignored.},
  % }
\fi

\endinput

==> tikzlibraryfeynman.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Pre-requisites
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
  arrows.meta,
  calc,
  decorations,
  decorations.markings,
  decorations.pathmorphing,
  decorations.pathreplacing,
  graphs,
  patterns,
  positioning,
  shapes.geometric,
}
\ifluatex
  \usetikzlibrary{
    graphdrawing
  }
  \usegdlibrary{
    circular,
    force,
    layered,
    trees
  }
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Miscellaneous functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@empty{}

%% Key Manager
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Setup the tikz-feynman key family
\pgfkeys{
  /tikzfeynman/.is family,
  /tikzfeynman/.search also={/tikz},
}

%% |\tikzfeynmanset| allows keys that belong with tikz-feynman to be easily set.
\def\tikzfeynmanset{\pgfqkeys{/tikzfeynman}}

%% Luatex Waring
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check if we are using luatex
\newif\iftikzfeynman@warn@luatex%
\tikzfeynmanset{
  warn luatex/.is if=tikzfeynman@warn@luatex,
  warn luatex=true,
}

\AtBeginDocument{
  \ifluatex\else
    \iftikzfeynman@warn@luatex
      \PackageWarning{tikz-feynman}{LuaTeX is required if you wish to have vertices automatically placed.  You can disable this warning by setting /tikzfeynman/warn luatex=false}
    \fi
  \fi
}

%% Version check
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check which version is expected and which is installed
\def\tikzfeynman@compat@parse#1.#2.#3\pgfeov{
  \edef\tikzfeynman@compat@major{#1}
  \edef\tikzfeynman@compat@minor{#2}
  \edef\tikzfeynman@compat@patch{#3}
  \edef\tikzfeynman@compat{#1.#2.#3}
}
\let\tikzfeynman@compat=\tikzfeynman@empty
\pgfkeyslet{/tikzfeynman/compat/.@cmd}{\tikzfeynman@compat@parse}
\ProcessPgfPackageOptions{/tikzfeynman}

\AtBeginDocument{
  \ifx\tikzfeynman@version\tikzfeynman@compat\else
    \ifx\tikzfeynman@compat\tikzfeynman@empty
      \PackageWarning{tikz-feynman}{Consider loading TikZ-Feynman with \string\usepackage[compat=\tikzfeynman@version]{tikz-feynman} so that you can be warned if TikZ-Feynman changes.}
    \else
      \ifx\tikzfeynman@compat@major\tikzfeynman@version@major
        \ifx\tikzfeynman@compat@minor\tikzfeynman@version@minor
          \ifx\tikzfeynman@compat@patch\tikzfeynman@version@patch\else
            \PackageInfo{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This should cause no issue.}
          \fi
        \else
          \PackageWarning{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This may change some diagrams.}
        \fi
      \else
        \PackageError{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  They are most likely incompatible.  Please download the appropriate version from jpellis.me/projects/tikz-feynman.}
      \fi
    \fi
  \fi
}

%% Override Lua code if necessary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@apply@patch#1{
  \directlua{require("tikzfeynman.patch.#1.lua")}
}

%% Version 3.0.0, 3.0.1 and 3.0.1a need to be patched.
\ifluatex
  \def\tikzfeynman@temp{3.0.0}
  \ifx\pgfversion\tikzfeynman@temp
    \tikzfeynman@apply@patch{3.0.0}
  \else
    \def\tikzfeynman@temp{3.0.1}
    \ifx\pgfversion\tikzfeynman@temp
      \tikzfeynman@apply@patch{3.0.1}
    \else
      \def\tikzfeynman@temp{3.0.1a}
      \ifx\pgfversion\tikzfeynman@temp
        \tikzfeynman@apply@patch{3.0.1}
      \fi
    \fi
  \fi
\fi

%% Feynman Environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Provide `\begin{feynman} ... \end{feynman}` within TikZ pictures.
\tikzaddtikzonlycommandshortcutlet\feynman\tikzfeynman@environment@feynman
\tikzaddtikzonlycommandshortcutlet\endfeynman\endtikzfeynman@environment@feynman

%% \begin{feynman}...\end{feynman}
\def\tikzfeynman@environment@feynman{%
  \pgfutil@ifnextchar[{\tikzfeynman@environment@feynman@opt}
  {\tikzfeynman@environment@feynman@opt[]}}

\def\tikzfeynman@environment@feynman@opt[#1]{%
  \begingroup
  %% Local overrides
  \let\tikz@@scan@fig=\tikzfeynman@scan@fig
  \let\tikzfeynman@orig@graph=\graph
  %% Local commands
  \let\vertex=\tikzfeynman@commands@vertex
  \let\diagram=\tikzfeynman@commands@diagram
  \let\graph=\tikzfeynman@commands@graph
  %% Opening hooks
  \scope
  \tikz@lib@ignore@sizetrue
  \tikzfeynman@tikz@search@tikzfeynman
  \pgfkeys{/tikzfeynman/every feynman@@,#1}
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman@@}%
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman}%
}

\def\endtikzfeynman@environment@feynman{%
  %% Closing hooks
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman}%
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman@@}%
  \endscope
  \endgroup
}

%% \feynmandiagram
\def\feynmandiagram{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt}
  {\feynmandiagram@opt[]}}
\def\feynmandiagram@opt[#1]{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt@opt[#1]}
  {\feynmandiagram@opt@opt[#1][#1]}}
\def\feynmandiagram@opt@opt[#1][#2]{%
  \tikz [/tikzfeynman/.cd,#1]
  \graph [/tikzfeynman/.cd,/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#2]}

%% Allow empty nodes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikzfeynmanallowemptynode
\newif\iftikzfeynmanvertex
\def\tikzfeynman@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
      {\iftikzfeynmanvertex%
         \tikzset{/tikzfeynman/every vertex@@}%
         \iftikzfeynmanallowemptynode%
         \else%
           \tikzset{/tikzfeynman/particle}%
         \fi%
       \fi%
       \tikz@fig@main{}}}}}}%}}

%% Include /tikzfeynman in the search path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@tikz@search@tikzfeynman{%
  \pgfkeys{/tikz/.unknown/.code=%
    \let\tikz@key\pgfkeyscurrentname%
    %% Is it a tikzfeynman key?
    \pgfkeys{/tikzfeynman/\tikz@key/.try={##1}}%
    \ifpgfkeyssuccess%
    \else%
      %% Is it a pgf key?
      \pgfkeys{/pgf/\tikz@key/.try={##1}}%
      \ifpgfkeyssuccess%
      \else%
        \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          %% this is a color!
          \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
          \edef\tikz@textcolor{\tikz@key}%
        \else%
          \pgfutil@doifcolorelse{\tikz@key}
          {%
            \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
            \edef\tikz@textcolor{\tikz@key}%
          }%
          {%
            %% Ok, second chance: This might be an arrow specification:
            \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
            \ifpgfutil@in@%
              %% Ah, an arrow spec!
              \expandafter\tikz@processarrows\expandafter{\tikz@key}%
            \else%
              %% Ok, third chance: A shape!
              \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
                \pgfkeys{/errors/unknown key/.expand
                once=\expandafter{\expandafter/\expandafter t\expandafter
                i\expandafter k\expandafter z\expandafter/\tikz@key}{##1}}%
              \else%
                \edef\tikz@shape{\tikz@key}%
              \fi%
            \fi%
          }%
        \fi%
      \fi%
    \fi%
  }
}


%% Vertex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Adapted from |\coordinate| code
\def\tikzfeynman@commands@vertex{
  \path \pgfextra{\tikzfeynmanallowemptynodetrue}
        \pgfextra{\tikzfeynmanvertextrue}
        node}

%% Diagram
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@diagram{\@ifstar
  \tikzfeynman@commands@diagram@star%
  \tikzfeynman@commands@diagram@nostar}

\def\tikzfeynman@commands@diagram@nostar{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@nostar@opt}
  {\tikzfeynman@commands@diagram@nostar@opt[]}}
\def\tikzfeynman@commands@diagram@nostar@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#1]}

\def\tikzfeynman@commands@diagram@star{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@star@opt}
  {\tikzfeynman@commands@diagram@star@opt[]}}
\def\tikzfeynman@commands@diagram@star@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Graph
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@graph{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@graph@opt}
  {\tikzfeynman@commands@graph@opt[]}}
\def\tikzfeynman@commands@graph@opt[#1]{%
  \PackageWarning{tikz-feynman}{It is not recommended to use \string\graph.  Use \string\diagram\space or \string\diagram* instead.}
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Optional argument in style key
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@key@opt#1[#2]#3\pgfeov{%
  \tikzfeynmanset{#1={[#2]#3}}}

%% Insertion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@insertion{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{insertion@@}}
  {\tikzfeynman@key@opt{insertion@@}[]}}
\pgfkeyslet{/tikzfeynman/insertion/.@cmd}{\tikzfeynman@insertion}

%% Momentum
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@momentum@std{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum@@}}
  {\tikzfeynman@key@opt{momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum/.@cmd}{\tikzfeynman@momentum@std}

\def\tikzfeynman@momentum@stdp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum'@@}}
  {\tikzfeynman@key@opt{momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum'/.@cmd}{\tikzfeynman@momentum@stdp}

\def\tikzfeynman@momentum@stdr{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum@@}}
  {\tikzfeynman@key@opt{reversed momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum/.@cmd}{\tikzfeynman@momentum@stdr}
\pgfkeyslet{/tikzfeynman/rmomentum/.@cmd}{\tikzfeynman@momentum@stdr}

\def\tikzfeynman@momentum@stdrp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum'@@}}
  {\tikzfeynman@key@opt{reversed momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum'/.@cmd}{\tikzfeynman@momentum@stdrp}
\pgfkeyslet{/tikzfeynman/rmomentum'/.@cmd}{\tikzfeynman@momentum@stdrp}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input tikzfeynman.keys.code.tex

\endinput
